Guaranteeing the \~O(AGM/OUT) Runtime for Uniform Sampling and OUT Size Estimation over Joins

We propose a new method for estimating the number of answers OUT of a small join query Q in a large database D, and for uniform sampling over joins. Our method is the first to satisfy all the following statements. - Support arbitrary Q, which can be either acyclic or cyclic, and contain binary and non-binary relations. - Guarantee an arbitrary small error with a high probability always in \~O(AGM/OUT) time, where AGM is the AGM bound OUT (an upper bound of OUT), and \~O hides the polylogarithmic factor of input size. We also explain previous join size estimators in a unified framework. All methods including ours rely on certain indexes on relations in D, which take linear time to build offline. Additionally, we extend our method using generalized hypertree decompositions (GHDs) to achieve a lower complexity than \~O(AGM/OUT) when OUT is small, and present optimization techniques for improving estimation efficiency and accuracy.

==> 00.revision_1st_round.tex <==
\newcommand{\metareviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Meta-Reviewer}}}
\newcommand{\reviewcomment}[2]{\vspace{0.5ex}\noindent\underline{\textbf{C#1:}} \textit{#2}\vspace{1pt}} %
\newcommand{\reviewremark}[2]{\vspace{0.5ex}\noindent\underline{\textbf{Additional Remark (#1):}} \textit{#2}\vspace{1pt}} %
\newcommand{\reviewrequiredchange}[1]{\vspace{0.5ex}\noindent\underline{\textbf{Required Change:}} \textit{#1}\vspace{1pt}} %
\newcommand{\reviewwriting}[1]{\vspace{0.5ex}\noindent\underline{\textbf{Inclusive Writing:}} \textit{#1}\vspace{1pt}} %
\newcommand{\response}[1]{\noindent\textbf{Response:} #1\color{black}} %

\newcommand{\revisionhl}[1]{\textcolor{blue}{#1}}
\newcommand{\reviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Reviewer #1}}} %
\newcommand{\orevisions}[1]{\vspace{2ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Other Revisions}}} %

\twocolumn

\noindent {\Large \bf Cover Letter for the 1st Round Comments}


\vspace{1ex}\noindent
We deeply appreciate all valuable comments from the first round of PODS 2023 and the chance to resubmit our revised paper to the second round. In our revised version, we have carefully addressed all questions and clarification requests. For convenience, the changes to the paper are colored in \revision{blue}.

%\coverletter{TBD: add (page, col, para)}

%We deeply appreciate your valuable comments. In our revised version, we have carefully addressed all questions and clarification requests.

%We are confident that our revised paper can address your valuable comments. The comments of the reviewers were very helpful in improving the quality of the paper. We hope our rebuttal will lead to your positive decision. Please refer to our response which helps clear the misunderstanding due to some presentation issues.

%============================================================================================================Meta Reviewer
\metareviewer\\

\reviewcomment{1}{The correctness concern asked by Reviewer 2.}

\response{We have clarified this concern which resulted from the misunderstanding of our $R_F$ notation in Algorithm \ref{alg:sampler} and omitted explantions in our proof of Lemma \ref{lemma:psmall} in equation (\ref{eq:reviewer2}). Please refer to our responses to [R2.C1-2].}

\reviewcomment{2}{The writing quality issues pointed out by all reviewers.}

\response{We have clarified all presentation issues by adding more explanations and removing ambiguities. Please refer to our responses to [R1.C1-4, R1.C7-9, R3.C2, R4.C1-2]. \coverletter{We have ensured this by asking two graduate students to read and confirm the accessibility and understandability of our revised manuscript.}}

Reviewer 3 suggested very recent papers about the approximate counting of conjunctive queries. We have added the discussions about an extension to conjunctive queries to strengthen our paper further.



%============================================================================================================REVIEWER 1
\reviewer{1}

We appreciate your comments about our presentation issues. We admit that we used some terminologies interchangeably if readers may understand from the context. For example, $P$ is a probability distribution, while $P(x)$ represents the probability of the value $x$. As per request, we have used the most suitable terminology and define operators and notations in Tables \ref{table:operators} and \ref{table:notations}. We have also removed all ambiguities in our revision.

\reviewcomment{1}{Joins (which are at the core of this paper) are not defined.}

\response{The first paragraph of \cref{sec:introduction} gives a formal definition of join we consider. Existing works (e.g., \cite{GJSampler, GenericJoin} in our revised paper) use the same definition as ours. We have also defined operators in Table \ref{table:operators}.}

%The definition is also clearer if we add explanations about operators (please refer to our response to C2).}

\reviewcomment{2}{Some operators (e.g. bowtie and uplus) were not defined, nor was a reference for a place that defines them given.}

\response{$\bowtie$ is a natural join operator \cite{PANDA, GenericJoin} widely used in previous work. $\uplus$ is a concatenation operator. For ease of reference, we have added Table \ref{table:operators} to describe the symbols used and their meanings.}

\reviewcomment{3}{Elements that are used in statements and explanations are not properly defined, rather they rely on using the same letter for the notation that was mentioned in previous sections in a different context. This is always confusing and sometimes really problematic. For example, in section 1.1, $P$ is both a probability and a distribution.}

\response{$P$ is a probability distribution, \coverletter{a mathematical function that gives the probabilities of events\footnote{\url{https://en.wikipedia.org/wiki/Probability_distribution}},} while $P(x)$ represents the probability (measure) of an event $x$. We have removed \coverletter{using $P$ as both a distribution and probability measure in \cref{subsec:introduction:previous}.}} %\coverletter{cite Introduction to Modern Statistics?}}

\reviewcomment{4}{Some notation, e.g. $F^*$ in section 1.2, I never found. It seems like the reader is expected to guess that whenever the letter $F$ is used, this means an edge/attribute. In Section 3.2, $\hyperedges_I$ under Alley wasn't defined.}

\response{We have defined notations in Table \ref{table:notations}. $F$ is always used as an edge, which is equivalent to a set of attributes as first explained in \cref{sec:introduction}. $F^*$ is a chosen edge from $\hyperedges$ under a criteria of each sampling-based estimator. For a set of edges $\hyperedges$ and a set of attributes $I$, $\hyperedges_I$ is defined as $\{F \in \hyperedges | F \cap I \neq \emptyset\}$, i.e., the set of edges in $\hyperedges$ which contain any attribute in $I$.}

\reviewcomment{5}{Some statements don't make much sense. Right before section 1.1: it is not clear why we would care about linear preprocessing for estimating join size (the runtime is larger than linear anyway) or what are online overheads.}

\response{We have revised the paragraph right before \cref{subsec:introduction:previous} 
\coverletter{that the sublinear time can be achieved for $\OUT$ sufficiently
large, especially when $\OUT$ is $\Omega(\IN^{\rho(\hypergraph)-1})$. \coverletter{For example, if $\OUT$ is $\Omega(\IN^{\rho(\hypergraph)})$, then the runtime becomes $\O(1)$.}
In approximating the $\OUT$ value, it is unnecessary to scan the inputs \coverletter{for each query} that requires $\O(\IN)$ time unlike the join processing.}
%Since the desired \emph{online} runtime for each query $\hypergraph$ is $\O(\frac{\IN^{\rho(\hypergraph)}}{\OUT})$, it can be smaller than $\O(\IN)$ if $\OUT$ is larger than $\O(\IN^{\rho(\hypergraph)-1})$.
%Please note that we solve the problem of approximating the $\OUT$ value, instead of enumerating all $\OUT$ number of join results. Therefore, $\O(\IN)$-time processing such as scanning the whole input data, may be unnecessary for each query.

Analogously, consider a simple sampling problem where we draw $n$ random samples from 0, ..., $N$-1. Some algorithms such as the classic Fisher-Yates method or sequential random sampling ([a] below) would always require linear preprocessing, i.e., the $O(N)$ preprocessing time. However, the algorithm in [b] supported by the well-known Weka library can draw $n$ random samples in $O(n)$ without the $O(N)$ preprocessing time. Please also refer to the last paragraph in \cref{sec:sampling} regarding why $T$ (or $\E[T]$) of \SSTE, \SUST, \GJSampler, and ours, is inversely proportional to $\OUT$.

\hfill % \break

\noindent [a] Vitter, J.S., 1987. An efficient algorithm for sequential random sampling. ACM transactions on mathematical software (TOMS), 13(1), pp.58-67.

\noindent [b]  Bui, D.N., 2015. Cachediff: Fast random sampling. arXiv preprint arXiv:1512.00501.

\hfill %\break

We would like to also note that we (and previous work \cite{SSTE, SUST, GJSampler}) require $\O(\IN)$-time \emph{offline} preprocessing to build indexes that support $\O(1)$-time operations such as semi-joins and sampling. Please refer to R4.C4 and our new section \cref{subsec:introduction:structure} that explains the underlying data structure and query (operation) model. This common $\O(\IN)$-time preprocessing is performed only once for a database, thus removed from our online runtime analysis. However, the $\O(\IN)$-time overhead we point out in \GJSampler must be done for \emph{each query}, thus must be included in its online runtime. This adds $+\IN$ term for sequenceable queries and $\coverletter{\times} \IN$ factor for non-sequenceable queries. 

%In that sense, Phrase 2) right before \cref{subsec:introduction:previous} states that \GJSampler requires either an $O(\IN)$ preprocessing (other than scanning the whole data) or overheads that result in an $O(\IN)$ factor, leading to $O(\frac{IN^{\rho(\hypergraph)+1}}{\OUT})$ time. 
}

\reviewcomment{6}{In section 1.1., it is said that \Alley solves approximate counting in $\O(\IN^\rho)$ time, but in this time you can compute the entire join.}

\response{\Alley indeed requires $\O(\IN^{\rho(\hypergraph)})$ time for approximate counting, which is an upper bound of join processing. This is a limitation of \Alley, compared to other asymptotically faster methods. However, the constant in the big-Oh notation decreases with the \coverletter{decreasing} branching factor $b$, as stated in Proposition \ref{prop:time:alley} in \cref{subsec:sampling:analysis}. \coverletter{The variance, however, increases with the decreasing $b$.} We also explained that \coverletter{increasing $b$ up to one} makes \Alley an instance of a join algorithm, resulting in zero error (zero variance).}

\reviewcomment{7}{In section 3.2 under \SSTE, it is not clear why it is equivalent that a center vertex $z$ is sampled and that an edge $e$ from $R$ is sampled.}

\response{\coverletter{In} the first approach, when we sample a center vertex $z$ from $\pi_A(R)$, $P(z) = |R \ltimes z|/|R|$ \coverletter{where $\ltimes$ is the semi-join operator. In} the second approach, when we first sample an edge $e$ from $R$ and let $z = \pi_A(e)$, there are $|R \ltimes z|$ edges in $R$ having $z$ as their projection onto $A$. \coverletter{Since} each edge is sampled with probability $1/|R|$, $P(z) = |R \ltimes z|/|R|$. We have added this explanation in \cref{appendix:decomposition} \coverletter{where $a_1$ and $R_{F_1}$ in \cref{appendix:decomposition} correspond to $z$ and $R$ here}.}

\reviewcomment{8}{Obscure phrasing: e.g. ``break the O(...) runtime'', ``keeps the output-sensitive bound'', ``a more generalized bound''.}

\response{Thanks for your detailed comments. We have removed all such obscure phrases. For example, we have removed ``break the O(...) runtime'' from the abstract and ``keeps the output-sensitive bound'' from the introduction. For ``a more generalized bound,'' we rewrote it to ``a generalized bound'' in \cref{subsec:introduction:ours} since the first desired bound $\O(\frac{AGM}{\OUT})$ is a specific instance of our generalized bound. The concept of generalizing bounds and widths has been used in previous work, e.g., Theorem 1.4 and Theorem 1.7 of \cite{PANDA}.}

\reviewcomment{9}{The introduction is quite technical and not readable for someone not already familiar with some notions such as fhtw and worst-case optimal algorithms.}

\response{We have revised whole introduction and added more background information about the AGM bound, fractional hypertree width, and worst-case optimal join, so that people unfamiliar with these concepts can read \coverletter{our paper} well. We also refer readers to the comprehensive survey (\cite{GenericJoin} in our paper) for more details about these concepts. This will help readers understand our paper even if they are unfamiliar with these notions.
We have ensured this by asking two graduate students who are not familiar with these notions to read and confirm the accessibility and understandability of our revised manuscript.}





%============================================================================================================REVIEWER 2
\reviewer{2}

Thanks very much for your comments. All of your concerns are due to the possibly confusing notation of $R_F$ in Algorithm \ref{alg:sampler} and omitted explanations in our proof of Lemma \ref{lemma:psmall} in equation (\ref{eq:reviewer2}), not due to any correctness issue. Please refer to our responses to your comments below.

\reviewcomment{1}{The results of \cite{GJSampler} are not correctly interpreted and stated (This is not a minor issue, since the sampling algorithm proposed in this paper is built on \cite{GJSampler}, using the same high-level framework with slightly different details):}


\hfill

\textit{\cite{GJSampler}: Random sampling and size estimation over cyclic joins}

\hfill

\textit{On page 4 for \GJSampler, in defining $P(s_I) = \frac{AGM(\hypergraph_{\sappend})}{AGM(\hypergraph_s)}$, it states that}

\hfill

\textit{$AGM(\hypergraph_s) = \prod_{F \in \hyperedges} |R_F|^{x_F}$}

\hfill

\textit{This is not correct, as $AGM(\hypergraph_s)$ is the AGM bound of the residual hypergraph after fixing the tuple $s$, where $s$ is the current sample. More specifically, suppose Algorithm \ref{alg:sampler} has processed attributes $\{v_1, v_2, ..., v_i\}$, then the sample $s$ is a tuple defined over attributes $\{v_1, v_2, ..., v_i\}$. The correct expression of $AGM(\hypergraph_s)$ is:}

\hfill

$AGM(\hypergraph_s) = \prod_{F \in \hyperedges} |R_F \ltimes s|^{x_F}$

\hfill

\textit{where a semi-join between $R_F$ and tuple $s$ is applied.
Please see page 5 of \url{https://www.cse.ust.hk/~yike/icdt20.pdf}.
The same issue applies to $AGM(\hypergraph_{s \uplus s_I})$.}

\textit{As it interprets the algorithm \cite{GJSampler} incorrectly, one step of the algorithm presented in Section 3.3 should be corrected as:}

\hfill

\textit{Uniformly sampling a row $t$ from $R_{F^*} \ltimes s$, instead of $R_{F^*}$}

\hfill

\textit{As it uses the incorrect formulation for $AGM(\hypergraph_s)$ and $AGM(\hypergraph_{\sappend})$, the proof of Lemma \ref{lemma:psmall} in Appendix \cref{appendix:proof} is totally messy.}

\response{The $AGM(\hypergraph_s)$ defined in \cite{GJSampler} is the same as the one in our paper. In Algorithm 2 of \cite{GJSampler}, $R_F$ is not given as a parameter but is fixed. \coverletter{However,} in Algorithm \ref{alg:sampler} of \coverletter{our original submission}, the $R_F$ was given as the second parameter, passing $\pi_J(R_F \ltimes s_I)$ (where $J$ is the set of unbounded attributes, $\hypernodes \setminus I$) as $R_F$ to the recursive call; $J = \hypernodes \setminus I$ was passed as $\hypernodes$ and $\hyperedges_{J,\pi} = \hyperedges_{\hypernodes \setminus I,\pi}$ was passed as $\hyperedges$. Please refer to R1.C4 and Table \ref{table:notations} for the definitions of $\hyperedges_J$ and $\hyperedges_{J,\pi}$. Note that \cite{GenericJoin} also uses this recursive formulation, where the input hypergraph $\hypergraph(\hypernodes, \hyperedges)$ changes at each recursive call. In conclusion, $R_F$ in our Algorithm \ref{alg:sampler} was essentially the same as $R_F \ltimes s$ in \cite{GJSampler}. Also, our formulation for $AGM(\hypergraph_s)$ was the same as that in \cite{GJSampler}. Therefore, our formulation, interpretation, and proof were correct.

To make this formulation consistent with \cite{GJSampler}, we have revised not only Algorithm \ref{alg:sampler} but also Algorithms \ref{alg:genericsampler}-\ref{alg:genericjoin} and related notation. Following \cite{GJSampler}, we have removed the parameter $R_F$ from these algorithms and revised $AGM(\hypergraph_s)$ accordingly. Thanks again for your comments.}

\reviewcomment{2}{Even if we consider the formulation they used
as a special case of the correct formulation when $s = \emptyset$, the proof is still wrong due to:}

\hfill

$\hyperedges_J = (\hyperedges_J \cap \hyperedges_I) \cup (\hyperedges_J - \hyperedges_I)$ instead of $\hyperedges_J = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$

\hfill

\textit{If the correctness of Lemma 2 cannot be guaranteed, then the algorithm is also incorrect, since it is impossible to keep a sample with a probability strictly larger than 1.}

\textit{Indeed, I agree with the authors that $\hyperedges = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$, but $\hyperedges_J = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$ is also used in the proof of Lemma 2 in the first equality of (18), which does not necessarily hold.}

\response{First, our formulation is correct for any $s$, from the response to C1. %Please refer to R1.C4 for our definition of $\hyperedges_I$ (also defined in our new Table \ref{table:notations}), which is $\{F \in \hyperedges | F \cap I \neq \emptyset\}$, the set of edges in $\hyperedges$ which contain any attribute in $I$.
%Then, from $V = I \cup J$ (i.e., $\{I, J\}$ is a partition of $V$ according to Line 3 of Algorithm 1), any edge in $E$ must contain an edge in $I$ or $J$, as explained in the proof of Lemma 2 in Appendix D. Therefore, $E = E_I \cup E_J$, which can be rewritten to $E_I \cup (E_J - E_I)$ for removing duplicate edges in $E_J$ that also appear in $E_I$. Thus, the correctness of Lemma 2 and the algorithm is guaranteed.
In our previous proof of Lemma \ref{lemma:psmall} where 
%$I$ and $J$ were disjoint partitions of $\hypernodes$,
\coverletter{$\{I, J\}$ was a partition of $\hypernodes$,}
we used $\hyperedges = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$ but not $\hyperedges_J = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$. When extending $\prod_{F \in \hyperedges_J} |R_F \ltimes s_I|^{x_F}$ to $\prod_{F \in \hyperedges_I} |R_F \ltimes s_I|^{x_F} \cdot \prod_{F \in \hyperedges_J - \hyperedges_I} |R_F \ltimes s_I|^{x_F}$ in our previous \coverletter{proof}, we used that $|R_F \ltimes s_I| = 1$ for any $F \in \hyperedges_I - \hyperedges_J$.

More simply, our proof works not only for the equality, $\prod_{F \in \hyperedges_J} |R_F \ltimes s_I|^{x_F}$ = $\prod_{F \in \hyperedges_I} |R_F \ltimes s_I|^{x_F} \cdot \prod_{F \in \hyperedges_J - \hyperedges_I} |R_F \ltimes s_I|^{x_F}$, but also for the inequality ($\leq$), $\prod_{F \in \hyperedges_J} |R_F \ltimes s_I|^{x_F} \leq \prod_{F \in \hyperedges_I} |R_F \ltimes s_I|^{x_F} \cdot \prod_{F \in \hyperedges_J - \hyperedges_I} |R_F \ltimes s_I|^{x_F}$, since our goal of the proof was to show LHS $\leq$ RHS.
In that sense, the inequality directly holds from the trivial $\hyperedges_J \subseteq \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$ and $|R_F \ltimes s_I| \geq 1$ for any $F \in \hyperedges_I - \hyperedges_J$.

We have made this clear in our revised \coverletter{proof}, where the notations are changed according to C1.
%One can easily reason why the first equality of (18) holds as follows. For the denominators, $\prod_{F \in E} |R_F|^{x_F} = \prod_{F \in E_I} |R_F|^{x_F} * \prod_{F \in E_J - E_I} |R_F|^{x_F} from E = E_I \cup (E_J - E_I)$. For the numerators, $\prod_{F \in E_J} |R_F \ltimes s_I|^{x_F} = \prod_{F \in E_I \cap E_J} |R_F \ltimes s_I|^{x_F} * \prod_{F \in E_J - E_I} |R_F \ltimes s_I|^{x_F} = \prod_{F \in E_I} |R_F \ltimes s_I|^{x_F} * \prod_{F \in E_J - E_I} |R_F \ltimes s_I|^{x_F}$. The last equality holds from $|R_F \ltimes s_I| = 1 for any F \in E_I - E_J$, since any such $F$ is a subset of $I$, resulting in $R_F \ltimes s_I = s_{I \cap F}$.
}

\pagebreak


%============================================================================================================REVIEWER 3
\reviewer{3}

\reviewcomment{1}{A minor issue is that the paper seems not aware of the results presented in:}

\hfill

\textit{[1] Marcelo Arenas, Luis Alberto Croquevielle, Rajesh Jayaram, Cristian Riveros:
When is approximate counting for conjunctive queries tractable? STOC 2021: 1015-1027.}

\hfill

\textit{An extension of this result (for fraction hypertree width) was recently presented in PODS 2022:}

\hfill

\textit{[2] Jacob Focke, Leslie Ann Goldberg, Marc Roth, Stanislav Zivný:
Approximately Counting Answers to Conjunctive Queries with Disequalities and Negations. PODS 2022: 315-324.}

\hfill

\textit{Both papers study an orthogonal line of research by solving the approximate counting and uniform sampling problem of CQ queries (i.e., join queries with projections). They show that both problems can be solved in PTIME for the class of CQ queries with bounded fractional hypertree width.}



\textit{The recent results in [1,2] can be considered orthogonal to the results in this paper, given that they considered projection and the current paper does not. Still, the authors should discuss this line of research and mention whether the results can be applied for projection or not.}



\response{We appreciate your comment about the introduction of the two recent, relevant papers. We have cited these important papers in \cref{subsec:introduction:previous}. They solve more general problems, approximate counting and almost uniform sampling for conjunctive queries. Regarding the projection, the join query we are considering is a full conjunctive query where all attributes are output or projection attributes.
Still, we could easily extended our algorithm to approximate counting and uniform sampling for join-project queries (a.k.a. conjunctive queries), following the same analysis of Section 3 in the \cite{GJSampler}. We explained this in \cref{sec:future} and \cref{appendix:conjunctive}.}


\reviewcomment{2}{Minor Comments}

\reviewcomment{2.1}{Page 1, Intro, line 6. ``$|Q| = \Join ... R_F$'' = ``$|Q| = |\Join ... R_f|$''}

\response{\coverletter{We have corrected this.}}

\reviewcomment{2.2}{Page 1, Intro, line 10. Say that $\rho(\hypergraph)$ is the fractional edge cover number.}

\response{\coverletter{We have added that $\rho(\hypergraph)$ is the fractional edge cover number.}}

\reviewcomment{2.3}{Page 1, Sec 1.1. Say what \SSTE stands for.} %SUST까지

\response{\coverletter{We have added what \SSTE and \SUST stand for.}}

\reviewcomment{2.4}{Page 2, Definition 2. It is not clear what you are defining in Definition 2. It does not sound like a definition but more like a desire.}

\response{\coverletter{We have specified that Definition 2 defines our goal.}}

\reviewcomment{2.5}{Page 2, after Definition 2. $AGM(\hypergraph)$ should be $AGM(\hypergraph, D)$, because it depends on the size of $D$.}

\response{The AGM bound indeed depends on the database $D$, however, $D$ is assumed fixed and thus omitted, and $AGM(\hypergraph)$ is typically used in previous papers (e.g., \cite{PANDA, GJSampler} in our paper).}

\reviewcomment{2.6}{Page 2, col 2, line -3. ``The AGM bound is tight ...; there exists a database D s.t. OUT = AGM(H)'' => you should add that ``asymptotically''. Even I remember that this happens with a log factor.}

\response{%Thanks for your detailed comments. We have addressed all these minor comments as per request. 
The log factor resides in the time complexity of worst-case optimal join algorithms, for example, the multi-way intersection in \GenericJoin (Algorithm 3 in \cite{GenericJoin} and Algorithm \ref{alg:genericjoin} in \cref{appendix:algorithm:genericjoin} of our paper) adds the log overhead. Please refer to R4.C4 and our new section \cref{subsec:introduction:structure} for the basic operations involving the log factor. However, $\OUT = AGM(\hypergraph)$ is satisfied without a log factor, thus the AGM bound is said to be a tight bound \cite{AGM, GenericJoin}. We have added these in the second paragraph of introduction.}




%============================================================================================================REVIEWER 4
\reviewer{4}

\reviewcomment{}{\coverletter{\textit{This paper presents a simple and elegant algorithmic framework for sampling from joins as well as query output size estimation (which are essentially the same problem). The following three results are most important:}}}

\coverletter{\textit{(1) It shows how to achieve O(AGM/OUT) for all queries, removing the technical condition in prior work [13].}}

\coverletter{\textit{(2) It shows how to drop the O(IN)-time preprocessing step, which was needed in [13].}}

\coverletter{\textit{(3) It generalizes to GHDs, improving for queries of low width.}}

\reviewcomment{1}{The writing should be improved. For instance, the key notion of $R_t$, which is used in stating the main result on (3), is only algorithmically defined, and it's buried in the description of Algorithm 2 and 3. It should have a more declarative, mathematical definition.}

\response{We have revised the paper and tested the accessibility and understandability of the revision with two graduate students who were unfamiliar with the key notions of the work. Please refer to our response to R1.C9. 
We provide the declarative meaning (i.e., intuitive semantics) of $R_t$ in \cref{subsec:generalized:sampling} as an approximate annotated relation of $\hypergraph_{G(t)}$ in Table \ref{table:notations}, and analyze $R_t$ mathematically in \cref{subsec:generalized:analysis} in order to explain the main result on (3).}
%We defined $R_t$ mathematically in \cref{subsec:generalized:sampling} and also provided its declarative meaning (i.e., intuitive semantics) as an approximate annotated relation of $\hypergraph_{G(t)}$ in Table \ref{table:notations}, \coverletter{in order to explain the main result on (3).}}

\reviewcomment{2}{Lemma 2 has $s$, the current sample, but its proof conveniently drops it.}

\response{We have included all dropped symbols in all our proofs.}

\reviewcomment{3}{When the query is acyclic, which is the special where each GHD bag has only one relation, $O(1)$ time can be achieved after $O(\IN)$-time preprocessing, see}

\hfill

\textit{Answering (Unions of) Conjunctive Queries using Random Access and Random-Order Enumeration, Nofar Carmeli, Shai Zeevi, Christoph Berkholz, Benny Kimelfeld, Nicole Schweikardt}

\hfill

\textit{Random Sampling over Joins Revisited. Zhuoyue Zhao, Robert Christensen, Feifei Li, Xiao Hu, and Ke Yi.}

\hfill

\textit{I wonder if this special case can also be incorporated into your framework. So far, your general GHD algorithm seems to be inferior to these results when the query is acyclic.}

\response{In \cref{appendix:algorithm:yan}, we have added explanations of \ExactWeight algorithm of the second paper that performs uniform sampling in $\O(1)$ time after $\O(\IN)$-time preprocessing, and the first paper as an extension of \ExactWeight for unions of acyclic conjunctive queries and sampling without replacement. We explained that our \GHDSampler can also perform uniform sampling in $\O(1)$ time after $\O(\IN)$-time preprocessing, by simple modifications of storing intermediate result sizes as \ExactWeight. In that sense, \GHDSampler is not inferior to \ExactWeight, but \ExactWeight can be regarded as a specific instance of \GHDSampler (with these modifications) for GHDs of singe-edge nodes and acylic joins. Therefore, extending \ExactWeight to perform uniform sampling over arbitrary GHDs and cyclic queries would be an interesting future work, which we have added in \cref{sec:future}.}

%SimpleAggroYannakakis can compute OUT in O(IN) time, but uniform sampling is not supported. To support uniform sampling after SimpleAggroYannakakis, we should compute the weights of subtrees as ExactWeights during SimpleAggroYannakakis.}


\reviewcomment{4}{You claim sub-linear time can be achieved for OUT sufficiently large. This relies on the availability of certain data structures. I think you at least need these operations: 1. edge/tuple sampling, 2. degree queries (this is needed to compute the residual AGM bound). 3. lookup queries. These can be supported by building hash tables, which takes linear time. It is OK to exclude the cost of building the hash tables, but you need to state this explicitly. Generally speaking, for sublinear-time algorithms, people should be very careful about the model, i.e., which queries are allowed. See e.g., \url{https://www.wisdom.weizmann.ac.il/~oded/PDF/pt-v3.pdf}.}

\response{\coverletter{Thanks a lot for your detailed comment.} We have added \cref{subsec:introduction:structure} to explain the underlying data structures and query (operation) model used in our paper and other worst-case optimal join algorithms \cite{GenericJoin, LeapFrog, NPRR} and sampling algorithms \cite{SSTE, GJSampler}. As you have noted, we assume a B-tree-like index for each relation to perform degree operations, access/lookup operations, existence operations, and sampling operations in $\O(1)$ time. However, the attribute order of the index must be consistent with the attribute order of join or sampling algorithms. We explained two solutions used in literature: 1) a mild assumption used in \cite{GenericJoin} that builds an index for each relation, following a global attribute order (which queries should also follow), and 2) building an index for every possible order of a relation to support arbitrary attribute orders of queries \cite{EmptyHeaded}.}

==> 00.revision_2nd_round.tex <==
\newcommand{\metareviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Meta-Reviewer}}}
\newcommand{\reviewcomment}[2]{\vspace{0.5ex}\noindent\underline{\textbf{C#1:}} \textit{#2}\vspace{1pt}} %
\newcommand{\reviewremark}[2]{\vspace{0.5ex}\noindent\underline{\textbf{Additional Remark (#1):}} \textit{#2}\vspace{1pt}} %
\newcommand{\reviewrequiredchange}[1]{\vspace{0.5ex}\noindent\underline{\textbf{Required Change:}} \textit{#1}\vspace{1pt}} %
\newcommand{\reviewwriting}[1]{\vspace{0.5ex}\noindent\underline{\textbf{Inclusive Writing:}} \textit{#1}\vspace{1pt}} %
\newcommand{\response}[1]{\noindent\textbf{Response:} #1\color{black}} %

\newcommand{\revisionhl}[1]{\textcolor{blue}{#1}}
\newcommand{\reviewer}[1]{\vspace{1ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Reviewer #1}}} %
\newcommand{\orevisions}[1]{\vspace{2ex}\vspace{0.5ex}\noindent\underline{\textbf{\large Other Revisions}}} %

\twocolumn

\noindent {\Large \bf Cover Letter for the 1st Round Comments}


\vspace{1ex}\noindent
We deeply appreciate all valuable comments from the first round of PODS 2023 and the chance to resubmit our revised paper to the second round. In our revised version, we have carefully addressed all questions and clarification requests. For convenience, the changes to the paper are colored in \second{blue}.

%\coverletter{TBD: add (page, col, para)}

%We deeply appreciate your valuable comments. In our revised version, we have carefully addressed all questions and clarification requests.

%We are confident that our revised paper can address your valuable comments. The comments of the reviewers were very helpful in improving the quality of the paper. We hope our rebuttal will lead to your positive decision. Please refer to our response which helps clear the misunderstanding due to some presentation issues.

%============================================================================================================Meta Reviewer
\metareviewer\\

\reviewcomment{1}{The correctness concern asked by Reviewer 2.}

\response{We have clarified this concern which resulted from the misunderstanding of our $R_F$ notation in Algorithm \ref{alg:sampler} and omitted explantions in our proof of Lemma \ref{lemma:psmall} in equation (\ref{eq:reviewer2}). Please refer to our responses to [R2.C1-2].}

\reviewcomment{2}{The writing quality issues pointed out by all reviewers.}

\response{We have clarified all presentation issues by adding more explanations and removing ambiguities. Please refer to our responses to [R1.C1-4, R1.C7-9, R3.C2, R4.C1-2]. \coverletter{We have ensured this by asking two graduate students to read and confirm the accessibility and understandability of our revised manuscript.}}

Reviewer 3 suggested very recent papers about the approximate counting of conjunctive queries. We have added the discussions about an extension to conjunctive queries to strengthen our paper further.



%============================================================================================================REVIEWER 1
\reviewer{1}

We appreciate your comments about our presentation issues. We admit that we used some terminologies interchangeably if readers may understand from the context. For example, $P$ is a probability distribution, while $P(x)$ represents the probability of the value $x$. As per request, we have used the most suitable terminology and define operators and notations in Tables \ref{table:operators} and \ref{table:notations}. We have also removed all ambiguities in our revision.

\reviewcomment{1}{Joins (which are at the core of this paper) are not defined.}

\response{The first paragraph of \cref{sec:introduction} gives a formal definition of join we consider. Existing works (e.g., \cite{GJSampler, GenericJoin} in our revised paper) use the same definition as ours. We have also defined operators in Table \ref{table:operators}.}

%The definition is also clearer if we add explanations about operators (please refer to our response to C2).}

\reviewcomment{2}{Some operators (e.g. bowtie and uplus) were not defined, nor was a reference for a place that defines them given.}

\response{$\bowtie$ is a natural join operator \cite{PANDA, GenericJoin} widely used in previous work. $\uplus$ is a concatenation operator. For ease of reference, we have added Table \ref{table:operators} to describe the symbols used and their meanings.}

\reviewcomment{3}{Elements that are used in statements and explanations are not properly defined, rather they rely on using the same letter for the notation that was mentioned in previous sections in a different context. This is always confusing and sometimes really problematic. For example, in section 1.1, $P$ is both a probability and a distribution.}

\response{$P$ is a probability distribution, \coverletter{a mathematical function that gives the probabilities of events\footnote{\url{https://en.wikipedia.org/wiki/Probability_distribution}},} while $P(x)$ represents the probability (measure) of an event $x$. We have removed \coverletter{using $P$ as both a distribution and probability measure in \cref{subsec:introduction:previous}.}} %\coverletter{cite Introduction to Modern Statistics?}}

\reviewcomment{4}{Some notation, e.g. $F^*$ in section 1.2, I never found. It seems like the reader is expected to guess that whenever the letter $F$ is used, this means an edge/attribute. In Section 3.2, $\hyperedges_I$ under Alley wasn't defined.}

\response{We have defined notations in Table \ref{table:notations}. $F$ is always used as an edge, which is equivalent to a set of attributes as first explained in \cref{sec:introduction}. $F^*$ is a chosen edge from $\hyperedges$ under a criteria of each sampling-based estimator. For a set of edges $\hyperedges$ and a set of attributes $I$, $\hyperedges_I$ is defined as $\{F \in \hyperedges | F \cap I \neq \emptyset\}$, i.e., the set of edges in $\hyperedges$ which contain any attribute in $I$.}

\reviewcomment{5}{Some statements don't make much sense. Right before section 1.1: it is not clear why we would care about linear preprocessing for estimating join size (the runtime is larger than linear anyway) or what are online overheads.}

\response{We have revised the paragraph right before \cref{subsec:introduction:previous} 
\coverletter{that the sublinear time can be achieved for $\OUT$ sufficiently
large, especially when $\OUT$ is $\Omega(\IN^{\rho(\hypergraph)-1})$. \coverletter{For example, if $\OUT$ is $\Omega(\IN^{\rho(\hypergraph)})$, then the runtime becomes $\O(1)$.}
In approximating the $\OUT$ value, it is unnecessary to scan the inputs \coverletter{for each query} that requires $\O(\IN)$ time unlike the join processing.}
%Since the desired \emph{online} runtime for each query $\hypergraph$ is $\O(\frac{\IN^{\rho(\hypergraph)}}{\OUT})$, it can be smaller than $\O(\IN)$ if $\OUT$ is larger than $\O(\IN^{\rho(\hypergraph)-1})$.
%Please note that we solve the problem of approximating the $\OUT$ value, instead of enumerating all $\OUT$ number of join results. Therefore, $\O(\IN)$-time processing such as scanning the whole input data, may be unnecessary for each query.

Analogously, consider a simple sampling problem where we draw $n$ random samples from 0, ..., $N$-1. Some algorithms such as the classic Fisher-Yates method or sequential random sampling ([a] below) would always require linear preprocessing, i.e., the $O(N)$ preprocessing time. However, the algorithm in [b] supported by the well-known Weka library can draw $n$ random samples in $O(n)$ without the $O(N)$ preprocessing time. Please also refer to the last paragraph in \cref{sec:sampling} regarding why $T$ (or $\E[T]$) of \SSTE, \SUST, \GJSampler, and ours, is inversely proportional to $\OUT$.

\hfill % \break

\noindent [a] Vitter, J.S., 1987. An efficient algorithm for sequential random sampling. ACM transactions on mathematical software (TOMS), 13(1), pp.58-67.

\noindent [b]  Bui, D.N., 2015. Cachediff: Fast random sampling. arXiv preprint arXiv:1512.00501.

\hfill %\break

We would like to also note that we (and previous work \cite{SSTE, SUST, GJSampler}) require $\O(\IN)$-time \emph{offline} preprocessing to build indexes that support $\O(1)$-time operations such as semi-joins and sampling. Please refer to R4.C4 and our new section \cref{subsec:introduction:structure} that explains the underlying data structure and query (operation) model. This common $\O(\IN)$-time preprocessing is performed only once for a database, thus removed from our online runtime analysis. However, the $\O(\IN)$-time overhead we point out in \GJSampler must be done for \emph{each query}, thus must be included in its online runtime. This adds $+\IN$ term for sequenceable queries and $\coverletter{\times} \IN$ factor for non-sequenceable queries. 

%In that sense, Phrase 2) right before \cref{subsec:introduction:previous} states that \GJSampler requires either an $O(\IN)$ preprocessing (other than scanning the whole data) or overheads that result in an $O(\IN)$ factor, leading to $O(\frac{IN^{\rho(\hypergraph)+1}}{\OUT})$ time. 
}

\reviewcomment{6}{In section 1.1., it is said that \Alley solves approximate counting in $\O(\IN^\rho)$ time, but in this time you can compute the entire join.}

\response{\Alley indeed requires $\O(\IN^{\rho(\hypergraph)})$ time for approximate counting, which is an upper bound of join processing. This is a limitation of \Alley, compared to other asymptotically faster methods. However, the constant in the big-Oh notation decreases with the \coverletter{decreasing} branching factor $b$, as stated in Proposition \ref{prop:time:alley} in \cref{subsec:sampling:analysis}. \coverletter{The variance, however, increases with the decreasing $b$.} We also explained that \coverletter{increasing $b$ up to one} makes \Alley an instance of a join algorithm, resulting in zero error (zero variance).}

\reviewcomment{7}{In section 3.2 under \SSTE, it is not clear why it is equivalent that a center vertex $z$ is sampled and that an edge $e$ from $R$ is sampled.}

\response{\coverletter{In} the first approach, when we sample a center vertex $z$ from $\pi_A(R)$, $P(z) = |R \ltimes z|/|R|$ \coverletter{where $\ltimes$ is the semi-join operator. In} the second approach, when we first sample an edge $e$ from $R$ and let $z = \pi_A(e)$, there are $|R \ltimes z|$ edges in $R$ having $z$ as their projection onto $A$. \coverletter{Since} each edge is sampled with probability $1/|R|$, $P(z) = |R \ltimes z|/|R|$. We have added this explanation in \cref{appendix:decomposition} \coverletter{where $a_1$ and $R_{F_1}$ in \cref{appendix:decomposition} correspond to $z$ and $R$ here}.}

\reviewcomment{8}{Obscure phrasing: e.g. ``break the O(...) runtime'', ``keeps the output-sensitive bound'', ``a more generalized bound''.}

\response{Thanks for your detailed comments. We have removed all such obscure phrases. For example, we have removed ``break the O(...) runtime'' from the abstract and ``keeps the output-sensitive bound'' from the introduction. For ``a more generalized bound,'' we rewrote it to ``a generalized bound'' in \cref{subsec:introduction:ours} since the first desired bound $\O(\frac{AGM}{\OUT})$ is a specific instance of our generalized bound. The concept of generalizing bounds and widths has been used in previous work, e.g., Theorem 1.4 and Theorem 1.7 of \cite{PANDA}.}

\reviewcomment{9}{The introduction is quite technical and not readable for someone not already familiar with some notions such as fhtw and worst-case optimal algorithms.}

\response{We have revised whole introduction and added more background information about the AGM bound, fractional hypertree width, and worst-case optimal join, so that people unfamiliar with these concepts can read \coverletter{our paper} well. We also refer readers to the comprehensive survey (\cite{GenericJoin} in our paper) for more details about these concepts. This will help readers understand our paper even if they are unfamiliar with these notions.
We have ensured this by asking two graduate students who are not familiar with these notions to read and confirm the accessibility and understandability of our revised manuscript.}





%============================================================================================================REVIEWER 2
\reviewer{2}

Thanks very much for your comments. All of your concerns are due to the possibly confusing notation of $R_F$ in Algorithm \ref{alg:sampler} and omitted explanations in our proof of Lemma \ref{lemma:psmall} in equation (\ref{eq:reviewer2}), not due to any correctness issue. Please refer to our responses to your comments below.

\reviewcomment{1}{The results of \cite{GJSampler} are not correctly interpreted and stated (This is not a minor issue, since the sampling algorithm proposed in this paper is built on \cite{GJSampler}, using the same high-level framework with slightly different details):}


\hfill

\textit{\cite{GJSampler}: Random sampling and size estimation over cyclic joins}

\hfill

\textit{On page 4 for \GJSampler, in defining $P(s_I) = \frac{AGM(\hypergraph_{\sappend})}{AGM(\hypergraph_s)}$, it states that}

\hfill

\textit{$AGM(\hypergraph_s) = \prod_{F \in \hyperedges} |R_F|^{x_F}$}

\hfill

\textit{This is not correct, as $AGM(\hypergraph_s)$ is the AGM bound of the residual hypergraph after fixing the tuple $s$, where $s$ is the current sample. More specifically, suppose Algorithm \ref{alg:sampler} has processed attributes $\{v_1, v_2, ..., v_i\}$, then the sample $s$ is a tuple defined over attributes $\{v_1, v_2, ..., v_i\}$. The correct expression of $AGM(\hypergraph_s)$ is:}

\hfill

$AGM(\hypergraph_s) = \prod_{F \in \hyperedges} |R_F \ltimes s|^{x_F}$

\hfill

\textit{where a semi-join between $R_F$ and tuple $s$ is applied.
Please see page 5 of \url{https://www.cse.ust.hk/~yike/icdt20.pdf}.
The same issue applies to $AGM(\hypergraph_{s \uplus s_I})$.}

\textit{As it interprets the algorithm \cite{GJSampler} incorrectly, one step of the algorithm presented in Section 3.3 should be corrected as:}

\hfill

\textit{Uniformly sampling a row $t$ from $R_{F^*} \ltimes s$, instead of $R_{F^*}$}

\hfill

\textit{As it uses the incorrect formulation for $AGM(\hypergraph_s)$ and $AGM(\hypergraph_{\sappend})$, the proof of Lemma \ref{lemma:psmall} in Appendix \cref{appendix:proof} is totally messy.}

\response{The $AGM(\hypergraph_s)$ defined in \cite{GJSampler} is the same as the one in our paper. In Algorithm 2 of \cite{GJSampler}, $R_F$ is not given as a parameter but is fixed. \coverletter{However,} in Algorithm \ref{alg:sampler} of \coverletter{our original submission}, the $R_F$ was given as the second parameter, passing $\pi_J(R_F \ltimes s_I)$ (where $J$ is the set of unbounded attributes, $\hypernodes \setminus I$) as $R_F$ to the recursive call; $J = \hypernodes \setminus I$ was passed as $\hypernodes$ and $\hyperedges_{J,\pi} = \hyperedges_{\hypernodes \setminus I,\pi}$ was passed as $\hyperedges$. Please refer to R1.C4 and Table \ref{table:notations} for the definitions of $\hyperedges_J$ and $\hyperedges_{J,\pi}$. Note that \cite{GenericJoin} also uses this recursive formulation, where the input hypergraph $\hypergraph(\hypernodes, \hyperedges)$ changes at each recursive call. In conclusion, $R_F$ in our Algorithm \ref{alg:sampler} was essentially the same as $R_F \ltimes s$ in \cite{GJSampler}. Also, our formulation for $AGM(\hypergraph_s)$ was the same as that in \cite{GJSampler}. Therefore, our formulation, interpretation, and proof were correct.

To make this formulation consistent with \cite{GJSampler}, we have revised not only Algorithm \ref{alg:sampler} but also Algorithms \ref{alg:genericsampler}-\ref{alg:genericjoin} and related notation. Following \cite{GJSampler}, we have removed the parameter $R_F$ from these algorithms and revised $AGM(\hypergraph_s)$ accordingly. Thanks again for your comments.}

\reviewcomment{2}{Even if we consider the formulation they used
as a special case of the correct formulation when $s = \emptyset$, the proof is still wrong due to:}

\hfill

$\hyperedges_J = (\hyperedges_J \cap \hyperedges_I) \cup (\hyperedges_J - \hyperedges_I)$ instead of $\hyperedges_J = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$

\hfill

\textit{If the correctness of Lemma 2 cannot be guaranteed, then the algorithm is also incorrect, since it is impossible to keep a sample with a probability strictly larger than 1.}

\textit{Indeed, I agree with the authors that $\hyperedges = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$, but $\hyperedges_J = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$ is also used in the proof of Lemma 2 in the first equality of (18), which does not necessarily hold.}

\response{First, our formulation is correct for any $s$, from the response to C1. %Please refer to R1.C4 for our definition of $\hyperedges_I$ (also defined in our new Table \ref{table:notations}), which is $\{F \in \hyperedges | F \cap I \neq \emptyset\}$, the set of edges in $\hyperedges$ which contain any attribute in $I$.
%Then, from $V = I \cup J$ (i.e., $\{I, J\}$ is a partition of $V$ according to Line 3 of Algorithm 1), any edge in $E$ must contain an edge in $I$ or $J$, as explained in the proof of Lemma 2 in Appendix D. Therefore, $E = E_I \cup E_J$, which can be rewritten to $E_I \cup (E_J - E_I)$ for removing duplicate edges in $E_J$ that also appear in $E_I$. Thus, the correctness of Lemma 2 and the algorithm is guaranteed.
In our previous proof of Lemma \ref{lemma:psmall} where 
%$I$ and $J$ were disjoint partitions of $\hypernodes$,
\coverletter{$\{I, J\}$ was a partition of $\hypernodes$,}
we used $\hyperedges = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$ but not $\hyperedges_J = \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$. When extending $\prod_{F \in \hyperedges_J} |R_F \ltimes s_I|^{x_F}$ to $\prod_{F \in \hyperedges_I} |R_F \ltimes s_I|^{x_F} \cdot \prod_{F \in \hyperedges_J - \hyperedges_I} |R_F \ltimes s_I|^{x_F}$ in our previous \coverletter{proof}, we used that $|R_F \ltimes s_I| = 1$ for any $F \in \hyperedges_I - \hyperedges_J$.

More simply, our proof works not only for the equality, $\prod_{F \in \hyperedges_J} |R_F \ltimes s_I|^{x_F}$ = $\prod_{F \in \hyperedges_I} |R_F \ltimes s_I|^{x_F} \cdot \prod_{F \in \hyperedges_J - \hyperedges_I} |R_F \ltimes s_I|^{x_F}$, but also for the inequality ($\leq$), $\prod_{F \in \hyperedges_J} |R_F \ltimes s_I|^{x_F} \leq \prod_{F \in \hyperedges_I} |R_F \ltimes s_I|^{x_F} \cdot \prod_{F \in \hyperedges_J - \hyperedges_I} |R_F \ltimes s_I|^{x_F}$, since our goal of the proof was to show LHS $\leq$ RHS.
In that sense, the inequality directly holds from the trivial $\hyperedges_J \subseteq \hyperedges_I \cup (\hyperedges_J - \hyperedges_I)$ and $|R_F \ltimes s_I| \geq 1$ for any $F \in \hyperedges_I - \hyperedges_J$.

We have made this clear in our revised \coverletter{proof}, where the notations are changed according to C1.
%One can easily reason why the first equality of (18) holds as follows. For the denominators, $\prod_{F \in E} |R_F|^{x_F} = \prod_{F \in E_I} |R_F|^{x_F} * \prod_{F \in E_J - E_I} |R_F|^{x_F} from E = E_I \cup (E_J - E_I)$. For the numerators, $\prod_{F \in E_J} |R_F \ltimes s_I|^{x_F} = \prod_{F \in E_I \cap E_J} |R_F \ltimes s_I|^{x_F} * \prod_{F \in E_J - E_I} |R_F \ltimes s_I|^{x_F} = \prod_{F \in E_I} |R_F \ltimes s_I|^{x_F} * \prod_{F \in E_J - E_I} |R_F \ltimes s_I|^{x_F}$. The last equality holds from $|R_F \ltimes s_I| = 1 for any F \in E_I - E_J$, since any such $F$ is a subset of $I$, resulting in $R_F \ltimes s_I = s_{I \cap F}$.
}

\pagebreak


%============================================================================================================REVIEWER 3
\reviewer{3}

\reviewcomment{1}{A minor issue is that the paper seems not aware of the results presented in:}

\hfill

\textit{[1] Marcelo Arenas, Luis Alberto Croquevielle, Rajesh Jayaram, Cristian Riveros:
When is approximate counting for conjunctive queries tractable? STOC 2021: 1015-1027.}

\hfill

\textit{An extension of this result (for fraction hypertree width) was recently presented in PODS 2022:}

\hfill

\textit{[2] Jacob Focke, Leslie Ann Goldberg, Marc Roth, Stanislav Zivný:
Approximately Counting Answers to Conjunctive Queries with Disequalities and Negations. PODS 2022: 315-324.}

\hfill

\textit{Both papers study an orthogonal line of research by solving the approximate counting and uniform sampling problem of CQ queries (i.e., join queries with projections). They show that both problems can be solved in PTIME for the class of CQ queries with bounded fractional hypertree width.}



\textit{The recent results in [1,2] can be considered orthogonal to the results in this paper, given that they considered projection and the current paper does not. Still, the authors should discuss this line of research and mention whether the results can be applied for projection or not.}



\response{We appreciate your comment about the introduction of the two recent, relevant papers. We have cited these important papers in \cref{subsec:introduction:previous}. They solve more general problems, approximate counting and almost uniform sampling for conjunctive queries. Regarding the projection, the join query we are considering is a full conjunctive query where all attributes are output or projection attributes.
Still, we could easily extended our algorithm to approximate counting and uniform sampling for join-project queries (a.k.a. conjunctive queries), following the same analysis of Section 3 in the \cite{GJSampler}. We explained this in \cref{sec:future} and \cref{appendix:conjunctive}.}


\reviewcomment{2}{Minor Comments}

\reviewcomment{2.1}{Page 1, Intro, line 6. ``$|Q| = \Join ... R_F$'' = ``$|Q| = |\Join ... R_f|$''}

\response{\coverletter{We have corrected this.}}

\reviewcomment{2.2}{Page 1, Intro, line 10. Say that $\rho(\hypergraph)$ is the fractional edge cover number.}

\response{\coverletter{We have added that $\rho(\hypergraph)$ is the fractional edge cover number.}}

\reviewcomment{2.3}{Page 1, Sec 1.1. Say what \SSTE stands for.} %SUST까지

\response{\coverletter{We have added what \SSTE and \SUST stand for.}}

\reviewcomment{2.4}{Page 2, Definition 2. It is not clear what you are defining in Definition 2. It does not sound like a definition but more like a desire.}

\response{\coverletter{We have specified that Definition 2 defines our goal.}}

\reviewcomment{2.5}{Page 2, after Definition 2. $AGM(\hypergraph)$ should be $AGM(\hypergraph, D)$, because it depends on the size of $D$.}

\response{The AGM bound indeed depends on the database $D$, however, $D$ is assumed fixed and thus omitted, and $AGM(\hypergraph)$ is typically used in previous papers (e.g., \cite{PANDA, GJSampler} in our paper).}

\reviewcomment{2.6}{Page 2, col 2, line -3. ``The AGM bound is tight ...; there exists a database D s.t. OUT = AGM(H)'' => you should add that ``asymptotically''. Even I remember that this happens with a log factor.}

\response{%Thanks for your detailed comments. We have addressed all these minor comments as per request. 
The log factor resides in the time complexity of worst-case optimal join algorithms, for example, the multi-way intersection in \GenericJoin (Algorithm 3 in \cite{GenericJoin} and Algorithm \ref{alg:genericjoin} in \cref{appendix:algorithm:genericjoin} of our paper) adds the log overhead. Please refer to R4.C4 and our new section \cref{subsec:introduction:structure} for the basic operations involving the log factor. However, $\OUT = AGM(\hypergraph)$ is satisfied without a log factor, thus the AGM bound is said to be a tight bound \cite{AGM, GenericJoin}. We have added these in the second paragraph of introduction.}




%============================================================================================================REVIEWER 4
\reviewer{4}

\reviewcomment{}{\coverletter{\textit{This paper presents a simple and elegant algorithmic framework for sampling from joins as well as query output size estimation (which are essentially the same problem). The following three results are most important:}}}

\coverletter{\textit{(1) It shows how to achieve O(AGM/OUT) for all queries, removing the technical condition in prior work [13].}}

\coverletter{\textit{(2) It shows how to drop the O(IN)-time preprocessing step, which was needed in [13].}}

\coverletter{\textit{(3) It generalizes to GHDs, improving for queries of low width.}}

\reviewcomment{1}{The writing should be improved. For instance, the key notion of $R_t$, which is used in stating the main result on (3), is only algorithmically defined, and it's buried in the description of Algorithm 2 and 3. It should have a more declarative, mathematical definition.}

\response{We have revised the paper and tested the accessibility and understandability of the revision with two graduate students who were unfamiliar with the key notions of the work. Please refer to our response to R1.C9. 
We provide the declarative meaning (i.e., intuitive semantics) of $R_t$ in \cref{subsec:generalized:sampling} as an approximate annotated relation of $\hypergraph_{G(t)}$ in Table \ref{table:notations}, and analyze $R_t$ mathematically in \cref{subsec:generalized:analysis} in order to explain the main result on (3).}
%We defined $R_t$ mathematically in \cref{subsec:generalized:sampling} and also provided its declarative meaning (i.e., intuitive semantics) as an approximate annotated relation of $\hypergraph_{G(t)}$ in Table \ref{table:notations}, \coverletter{in order to explain the main result on (3).}}

\reviewcomment{2}{Lemma 2 has $s$, the current sample, but its proof conveniently drops it.}

\response{We have included all dropped symbols in all our proofs.}

\reviewcomment{3}{When the query is acyclic, which is the special where each GHD bag has only one relation, $O(1)$ time can be achieved after $O(\IN)$-time preprocessing, see}

\hfill

\textit{Answering (Unions of) Conjunctive Queries using Random Access and Random-Order Enumeration, Nofar Carmeli, Shai Zeevi, Christoph Berkholz, Benny Kimelfeld, Nicole Schweikardt}

\hfill

\textit{Random Sampling over Joins Revisited. Zhuoyue Zhao, Robert Christensen, Feifei Li, Xiao Hu, and Ke Yi.}

\hfill

\textit{I wonder if this special case can also be incorporated into your framework. So far, your general GHD algorithm seems to be inferior to these results when the query is acyclic.}

\response{In \cref{appendix:algorithm:yan}, we have added explanations of \ExactWeight algorithm of the second paper that performs uniform sampling in $\O(1)$ time after $\O(\IN)$-time preprocessing, and the first paper as an extension of \ExactWeight for unions of acyclic conjunctive queries and sampling without replacement. We explained that our \GHDSampler can also perform uniform sampling in $\O(1)$ time after $\O(\IN)$-time preprocessing, by simple modifications of storing intermediate result sizes as \ExactWeight. In that sense, \GHDSampler is not inferior to \ExactWeight, but \ExactWeight can be regarded as a specific instance of \GHDSampler (with these modifications) for GHDs of singe-edge nodes and acylic joins. Therefore, extending \ExactWeight to perform uniform sampling over arbitrary GHDs and cyclic queries would be an interesting future work, which we have added in \cref{sec:future}.}

%SimpleAggroYannakakis can compute OUT in O(IN) time, but uniform sampling is not supported. To support uniform sampling after SimpleAggroYannakakis, we should compute the weights of subtrees as ExactWeights during SimpleAggroYannakakis.}


\reviewcomment{4}{You claim sub-linear time can be achieved for OUT sufficiently large. This relies on the availability of certain data structures. I think you at least need these operations: 1. edge/tuple sampling, 2. degree queries (this is needed to compute the residual AGM bound). 3. lookup queries. These can be supported by building hash tables, which takes linear time. It is OK to exclude the cost of building the hash tables, but you need to state this explicitly. Generally speaking, for sublinear-time algorithms, people should be very careful about the model, i.e., which queries are allowed. See e.g., \url{https://www.wisdom.weizmann.ac.il/~oded/PDF/pt-v3.pdf}.}

\response{\coverletter{Thanks a lot for your detailed comment.} We have added \cref{subsec:introduction:structure} to explain the underlying data structures and query (operation) model used in our paper and other worst-case optimal join algorithms \cite{GenericJoin, LeapFrog, NPRR} and sampling algorithms \cite{SSTE, GJSampler}. As you have noted, we assume a B-tree-like index for each relation to perform degree operations, access/lookup operations, existence operations, and sampling operations in $\O(1)$ time. However, the attribute order of the index must be consistent with the attribute order of join or sampling algorithms. We explained two solutions used in literature: 1) a mild assumption used in \cite{GenericJoin} that builds an index for each relation, following a global attribute order (which queries should also follow), and 2) building an index for every possible order of a relation to support arbitrary attribute orders of queries \cite{EmptyHeaded}.}

==> 04.outdated.tex <==
%\redtext{Using a fancy idea from linear programming and simple modifications, in Section \ref{sec:decomposition} we remove this assumption and show that Lemma \ref{lemma:decomposition} holds for labeled graphs as well.}


%\SSTE and other sampling-based estimators basically use the Horvits-Thompson (HT) estimator \cite{} to compute the estimate $\widehat{\#H}$ from the samples $\Samples$ as (\ref{eq:HT}). If a sample $p$ of $H$ is an embedding of $H$ (i.e., $p \in \Matches$), it results in a nonzero estimate $w(p) \coloneqq \frac{1}{P(p)}$, the inverse of probability sampling $p$. Otherwise if $p \not\in \Matches$, it results in zero estimate. The unbiasedness is guaranteed by all HT estimators. 


%\begin{equation}\label{eq:HT}
%\widehat{\#H} = \frac{1}{|\Samples|} \sum_{p \in \Samples}{w(p) \cdot \I[p \in \Matches]}
%\end{equation}


%A more detailed equation of \SSTE involving query decomposition is (\ref{eq:decomposition}). Let $c_1, c_2, ..., c_k$ the $k$ components (odd cycles and stars) of $H$ that are arbitrarily ordered.

%\begin{equation}\label{eq:decomposition}
%\begin{split}
%    \widehat{\#H} = \frac{1}{|\Samples_1|} \sum_{p_1 \in \Samples_1} \frac{1}{|\Samples_2|} \sum_{p_2 \in \Samples_2} ... \frac{1}{|\Samples_k|} \sum_{p_k \in \Samples_k} w(p_1, p_2, ..., p_k) \cdot \\
%    \I[(p_1, p_2, ..., p_k) \text{ forms an embedding of } H]
%\end{split}
%\end{equation}


%After decomposing $H$ into $k$ components (odd cycles and stars) using Lemma \ref{lemma:decomposition}, 


%\SSTE \cite{SSTE} samples a potential copy $p_i$ from $G$ for each $c_i$. Then, it checks whether these potential copies or samples for all components form an embedding of $H$, by checking 1) each $p_i$ is an embedding of $c_i$ and 2) $p_i$'s are connected by data edges, i.e., edges that should be matched to query edges $E(H) \setminus$SUPP($x^*$). 
%Here, the size of each $\Samples_i$ ($i > 1$) is determined by $p_{i-1}$ but not $\Samples_i$ itself, indicating that the sample spaces $\Samples_i$'s are independent. Since sampling each $p_i$ is also independent, we can rewrite (\ref{eq:decomposition}) into (\ref{eq:decomposition2}). 
%\SSTE chooses $|\Samples_i|$ ($i > 1$) in order to maintain an upper bound of variance on each partial sum $\frac{w(p_{i-1})}{|\Samples_{i}|} \sum_{p_{i} \in \Samples_{i}} ... \sum_{p_k \in \Samples_k} w(p_k) \cdot \I$. We call it \emph{branching}.



%\begin{equation}\label{eq:decomposition2}
%\begin{split}
%    \widehat{\#H} = \frac{1}{|\Samples_1|} \sum_{p_1 \in \Samples_1} \frac{w(p_1)}{|\Samples_2|} \sum_{p_2 \in \Samples_2} ... \frac{w(p_{k-1})}{|\Samples_k|} \sum_{p_k \in \Samples_k} w(p_k) \cdot \\
%    \I[(p_1, p_2, ..., p_k) \text{ forms an embedding of } H]
%\end{split}
%\end{equation}


%However, this does not reveal the importance of decomposition into odd cycles and stars since it works for any sampling methods. 


%To recursively bound the variance of each partial sum, \SSTE uses a fact that the projection of an optimal edge cover found by Lemma \ref{lemma:decomposition} onto a subquery $H_{i} \coloneqq \cup_{j \geq i}{c_j}$, is also an optimal edge cover of $H_i$. As a result, the variances are expressed with $AGM(H_i)$ terms. See \cite{SSTE} for more details.

%any subquery $H'$ with subsets of odd cycles and stars, is also an optimal edge cover of $H'$. Then, an upper bound can be recursively expressed via AGM-related term.



%A projection of this optimal edge cover of H onto a subquery H’ 
%(with odd cycles & stars) is also an optimal edge cover of H’
%The proofs for theoretical bounds are based on the induction hypothesis 
%that the solution of H’ is a part of the solution of H


%In detail, to maintain the upper bound of the sampling variance, 

%This works in a recursive manner, i.e., it arbitrarily orders all components, and 


%\section{Decomposition for Labeled Graphs} \label{sec:decomposition}


%We show that Lemma \ref{lemma:decomposition} holds for labeled graphs with varying $|R_F|$ for $F \in \hyperedges$ in (\ref{eq:agm}), and extend \SSTE to labeled graphs. 








\iffalse

\begin{equation}
\begin{split}
=& \, |R|^n \sum_{s_I} \frac{\I[s_I] }{k} \Var\Big[\frac{ \I[s_{J_1}] Z_{\hypergraph_{J_2}} }{P(s_{J_1})}\Big]  \\
\leq & \, |R|^n \sum_{s_I} \frac{\I[s_I] \I[s_{J_1}] |R \ltimes \{a_1\}|^2 }{k} \E[ Z^2_{\hypergraph_{J_2}}]  \\
= & \, |R|^n \sum_{s_I} \frac{\I[s_I] \I[s_{J_1}] |R \ltimes \{a_1\}| }{k} \sum_{s_{J_1}} Z^2_{\hypergraph_{J_2}}
\leq & \, |R|^n \sum_{s_I} \frac{\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F] }{k} \E[Z^2_{\hypergraph_J}(s_J)] \\
= & \, |R|^n \sum_{s_I} \frac{\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F] }{k} \sum_{s_J} \frac{1}{|R \ltimes \{a_1\}|} Z^2_{\hypergraph_J}(s_J) \\
= & \, |R|^n \sum_{s_I} \frac{\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F] }{k} \sum_{s_J} |R \ltimes \{a_1\}| \\
 & \cdot \I[s_J \in \Join_{F \in \hyperedges_J} \pi_J (R_F \ltimes s_I)] \\
= & |R|^{n+\frac{1}{2}}  \sum_{s_I} \sum_{s_J} \I[s_I] \I[s_J] \\
= & |R|^{n+\frac{1}{2}} \OUT = AGM(\hypergraph) \cdot \OUT \,\,\, (\text{Lemma \ref{lemma:decomposition}}).
\end{split}
\end{equation}


\begin{equation}
\begin{split}
\Var[&Z_\hypergraph] \\
=& \, \frac{1}{k} \Var[Z_\hypergraph(s_I)] = \frac{1}{k} \Var\Big[\frac{\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F]}{P(s_I)}\Big] \\
=& \, \frac{|\SampleSpace_I|^2}{k} \Var[\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F]] \\
\leq & \frac{|\SampleSpace_I|^2}{k} \E[\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F]^2] \\
=& \, \frac{|\SampleSpace_I|^2}{k} \sum_{s_I \in \SampleSpace_I} P(s_I) \I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F] \\
=& \,  \frac{|\SampleSpace_I|}{k} \OUT = \sqrt{|R|} \OUT.
\end{split}
\end{equation}


For the base case, $I = \hypernodes$ is either $\{X\}$ for an attribute $X$ of an odd cycle $C$, or $n$ vertices of a star $S$ (see Section \ref{subsec:overview}). 
In the first case, 
\begin{equation}
\begin{split}
\Var[&Z_\hypergraph] \\
=& \, \frac{1}{k} \Var[Z_\hypergraph(s_I)] = \frac{1}{k} \Var\Big[\frac{\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F]}{P(s_I)}\Big] \\
=& \, \frac{|\SampleSpace_I|^2}{k} \Var[\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F]] \\
\leq & \frac{|\SampleSpace_I|^2}{k} \E[\I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F]^2] \\
=& \, \frac{|\SampleSpace_I|^2}{k} \sum_{s_I \in \SampleSpace_I} P(s_I) \I[s_I \in \Join_{F \in \hyperedges_I} \pi_I R_F] \\
=& \,  \frac{|\SampleSpace_I|}{k} \OUT = \sqrt{|R|} \OUT.
\end{split}
\end{equation}

$k = \frac{}{}$


If $I$ forms an odd cycle, let $\textbf{e} = \{e_1, e_2, ..., e_n\}$ where $e_i$ is defined in Section \ref{subsec:overview}.
Then, $\Var[Z_\hypergraph] = \E[\Var[Z_\hypergraph | \textbf{e}]]  + \Var[\E[Z_\hypergraph | \textbf{e}]]$ from the law of total variance.
For the first term,


\begin{equation}
\begin{split}
\E[\Var[Z_\hypergraph | \textbf{e}]] 
= \sum_{\textbf{e} \in R^n} P(e) \Var[Z_\hypergraph | \textbf{e}] 
= \frac{1}{|R|^n} \sum_{\textbf{e} \in R^n} \frac{1}{k} \Var[Z_\hypergraph | \textbf{e}]
\end{split}
\end{equation}


$k = \ceil{\frac{\min(|R \ltimes \{a_1\}|, |R \ltimes \{b_1\}|)}{\sqrt{|R|}}}$. WLOG, let $|R \ltimes \{a_1\}| \leq |R \ltimes \{b_1\}|$. 

\fi








\iffalse
\begin{algorithm} [htb]
\caption{{\EnumerateTuples}($\hypergraph = (\hypernodes, \hyperedges)$, $\{R_F | F \in \hyperedges\}$)} \label{alg:enumeratetuples}
\small{
    \KwIn{Hypergraph $\hypergraph$ and relations $R_F$ for each $F \in \hyperedges$}
    
    $Q \leftarrow \emptyset$ \\
    
    Pick $I$ arbitrarily such that $|I| = 1$, $I \subset \hypernodes$ \\
    $F^* \leftarrow \argmin_{F \in \hyperedges_I}|R_F|$ \\ %semi-join included
    $\hypergraph_{-I} \leftarrow (\hypernodes \setminus I, \{ \pi_{\hypernodes \setminus I}(F) | F \in \hyperedges_{\hypernodes \setminus I} \})$ \\

    \ForEach{$t_I \in \pi_{I}(R_{F^*})$}
    {
        $Q \leftarrow Q \cup \{t_I\} \times \EnumerateTuples(\hypergraph_{-I}, \{\pi_{\hypernodes \setminus I}(R_F \ltimes t_I) | F \in  \hyperedges_{\hypernodes \setminus I}\})$ \\
    }
    
    \Return $Q$ \\
}
\end{algorithm}
\fi

\begin{algorithm} [htb]
\caption{{\SamplingEstimator}($\hypergraph = (\hypernodes, \hyperedges)$, $\{R_F|F \in \hyperedges\}$, $S$, $\{x_F | F \in \hyperedges\}$, \redtext{$\leaves$})} \label{alg:samplingestimator}
\small{
    \KwIn{Hypergraph $\hypergraph$, relations $R_F$ for each $F \in \hyperedges$, sample size $S$, fractional edge cover $\{x_F\}$, \redtext{and leaf relations $\leaves$}}
    
    Pick $I$ arbitrarily such that $|I| = 1$, $I \subset \hypernodes$ \\
    $F^* \leftarrow \argmin_{F \in \hyperedges_I}|R_F|$ \\ %semi-join included
    \If{$|R_{F^*}| = 0$}
    {
        \Return 0 \\
    }
    
    $\Samples_{I} \leftarrow $ uniform independent samples from $\pi_{I}(R_{F^*})$ with $|\Samples_{I}| = S$ \\
    
    \If{$|\hypernodes| = 1$}
    {
        \Return $\frac{|R_{F^*}|}{|\Samples_I|} \sum_{s_I \in \Samples_I}\I[s_I \in R_F : \forall F \in \hyperedges] \redtext{\prod_{F \in \leaves} |R_F \ltimes s_I|}$ \\
    }
    
    %Pick $I$ arbitrarily such that $1 \leq |I| < |\hypernodes|$ \\
    $\hypergraph_{-I} \leftarrow (\hypernodes \setminus I, \{ \pi_{\hypernodes \setminus I}(F) | F \in \hyperedges_{\hypernodes \setminus I} \})$ \\

    %Arbitrarily order vertices
    
    %$k \leftarrow s \mapsto \ceil{|\pi_{I}(R_{F^*})|  \frac{ \prod_{F \in \hyperedges_{\hypernodes \setminus I} }{|R_F \ltimes s|^{x_F}} }{ \prod_{F \in \hyperedges}{|R_F|^{x_F}} }}$ \\
    $k \leftarrow s \mapsto \ceil{|\pi_{I}(R_{F^*})|  \frac{AGM(\hypergraph_{-I})}{AGM(\hypergraph)}}$ \\
    
    
    \Return $\frac{|\pi_{I}(R_{F^*})|}{|\Samples_I|} \sum_{s_I \in \Samples_I} \I[s_I \in \pi_I(R_F) : \forall F \in \hyperedges_I] \cdot$
    $\SamplingEstimator(\hypergraph_{-I}, \{\pi_{\hypernodes \setminus I}(R_F \ltimes s_I) | F \in \hyperedges_{\hypernodes \setminus I}\}, k(s_I), \{x_F | F \in \hyperedges_{\hypernodes \setminus I}\}, \redtext{\leaves})$ \\
}
\end{algorithm}




















\iffalse

%\begin{definition2}
%\vspace*{-0.2cm}
%\label{def:approximation}
%For an error bound $\epsilon$, a confidence $\mu \in (0,1)$, and a true value $T$, if the random variable for the estimate $Z$ satisfies $P(\abs{Z-T} \geq \epsilon \cdot T) \leq \mu$, then the estimation is a $(1\pm\epsilon)$-approximation of $T$.
%\end{definition2}


\redtext{Need to define $Q^1$, $\hypergraph^1$, $G(\GHD)$, $\GHD(x)$ for an attribute $x$ as the subtree of $\GHD$ of nodes $t$ having $x \in \bag(t)$.}

\begin{theorem}\label{theorem:fhtw}
For arbitrary join query $Q = \hypergraph$ and GHD ($\GHD, \bag$) of $\hypergraph$, $\GHDSampler$ performs $(1\pm\epsilon)$-approximation of $|Q^1|$ in expected \redtext{$\DataO(\frac{IN^{fhtw(\GHD, \hypergraph)}}{|Q^1|^{1/|\hypernodes_\GHD|}})$} time. % where $m = \max_{x \in G(\GHD)} |\hypernodes_{\GHD(x)}|$.
%There exists a randomized algorithm that given a precision parameterε∈(0,1),a subgraphH, and a query access to the input graphG, with high probability outputs a(1±ε)approximation to the number of occurrences ofHinG, denoted by#H, using:
\end{theorem}

The proof for unbiasedness is straightforward. Each call to \SamplingEstimator at Line \ref{alg:genericsampler:sampler} of Algorithm \ref{alg:genericsampler} returns an unbiased estimate for $\hypergraph_{-G}$ given $g$. Therefore, each node $t \in \hypernodes_\GHD$ receives a relation $R_t$ with unbiased estimates for $\sum_{\bag(t) \setminus G(t)} \hypergraph^1_t$ (each tuple in $\hypergraph^1_t$ is a join result of $\hypergraph_t$ with annotation one). As a result, \GHDSampler returns an unbiased estimate of $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} \sum_{\bag(t) \setminus G(t)} \hypergraph^1_t$ = $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \sum_{\cup_{t \in \hypernodes_\GHD} \bag(t) \setminus G(t)} \Join_{t \in \hypernodes_\GHD} \hypergraph^1_t$ = $\sum_{\cup_{t \in \hypernodes_\GHD} \bag(t)} \Join_{t \in \hypernodes_\GHD} \hypergraph^1_t$ = $|Q^1|$.


Therefore, we focus on the variance and runtime. 

\begin{proposition2}\label{proposition:genericsampler:time}
For any $t \in \hypernodes_\GHD$, if we set $k = |\hypernodes| \, AGM(\hypergraph_{-G})$ for each tuple $g \in \hypergraph^1_G$, the expected runtime for \GenericSampler is $\DataO(AGM(\hypergraph))$.
\end{proposition2}

\begin{proof}
Line \ref{alg:genericsampler:sampler} of Algorithm \ref{alg:genericsampler} takes $\DataO(AGM(\hypergraph_G))$ where $AGM(\hypergraph_G) \leq AGM(\hypergraph)$ from the node-monotonicity of $AGM$ \cite{AJAR}.
The expected runtime of Lines 5-7 is $\sum_{g \in \hypergraph^1_G} AGM(\hypergraph_{-G}))$ from Proposition \ref{proposition:time}, which is less than $AGM(\hypergraph)$ from the query decomposition lemma of \cite{GenericJoin}.
Since the other lines take $\DataO(1)$, the expected runtime of Algorithm \ref{alg:genericsampler} is $\DataO(AGM(\hypergraph))$ as desired.
\end{proof}


\begin{proposition2}\label{proposition:ghdsampler:time}
For each $t \in \hypernodes_\GHD$ and $\hypergraph_t = (\hypernodes, \hyperedges)$, if we use the same $k$ from Proposition \ref{proposition:genericsampler:time}, the expected runtime for \GHDSampler is $\DataO(IN^{fhtw(\GHD, \hypergraph)})$.
\end{proposition2}

The proof is straightforward. Line \ref{alg:ghdsampler:generic} of Algorithm \ref{alg:ghdsampler} takes expected $\DataO(\max_{t \in \hypernodes_\GHD} AGM(\hypergraph_t))$ from Proposition \ref{proposition:genericsampler:time}. Line \ref{alg:ghdsampler:yan} takes $\DataO(IN + OUT)$ \cite{AJAR} where $IN = \DataO(\max_{t \in \hypernodes_\GHD} AGM(\hypergraph_t))$ and $OUT = 1$. Therefore, the expected runtime of \GHDSampler is $\DataO(\max_{t \in \hypernodes_\GHD} AGM(\hypergraph_t)) = \DataO(IN^{fhtw(\GHD, \hypergraph)})$.


\begin{proposition2}\label{proposition:ghdsampler:variance}
For each $t \in \hypernodes_\GHD$ and $\hypergraph_t = (\hypernodes, \hyperedges)$, if we use the same $k$ from Proposition \ref{proposition:genericsampler:time}, $\Var[Z_\hypergraph] \leq |\hypergraph^1|$ (= $|Q^1|$) for the estimate $Z_\hypergraph$ of \GHDSampler.
\end{proposition2}


\begin{proof}
$\Var[Z_\hypergraph] = \Var[\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R_t]$ where $R_t$ is the result of \GenericSampler annotated with $Z[t_{G(t)}]$'s, as in the analysis for the unbiasedness of $Z_\hypergraph$. 

%We can compute $\Var[Z_\hypergraph]$ from $\Var[Z[g(t)]]$ (Line 6 of Algorithm \ref{alg:genericsampler}) for each GHD node $t \in \hypernodes_\GHD$.
Since all $Z[g]$'s are mutually independent, even across different GHD nodes, $\Var[Z[g] + Z[t'_{G}]]$ = $\Var[Z[g]] + \Var[Z[t'_{G}]]$ and $\Var[Z[g \Join t'_{G'}]]$ = $\Var[Z[g] \times Z[t'_{G'}]]$ = $\Var[Z[g]] \times \Var[Z[t'_{G'}]]$ for any $g$, $t'_{G}$, and $t'_{G'}$ ($G \cap G' \neq \emptyset$). Therefore, as $Z[g]$ was the annotation for $g$ when estimating $|Q^1|$, we can regard $\Var[Z[g]]$ as the annotation for $g$ when calculating $\Var[Z_\hypergraph]$. We denote $R^{\Var}_t$ as $R_t$ whose annotations are replaced from $Z[g]$'s to $\Var[Z[g]]$'s.

\redtext{Need to define $\hypergraph[tuple]$ or $Q[tuple]$.}

We then calculate $\Var[Z_\hypergraph]$ as follows.
$\Var[\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R_t]$ = $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R^{\Var}_t$ $\leq$ 
$\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} \sum_{\bag(t) \setminus G(t)} \hypergraph^1_t$ = $|Q^1|$. The inequality holds from Proposition \ref{proposition:var}, $\Var[Z[g]] \leq |\Join_{F \in \hyperedges_{\hypernodes \setminus G}} \pi_{\hypernodes \setminus G}(R_F \ltimes g)| = \sum_{\hypernodes \setminus G} \hypergraph^1_t[g] = \sum_{\bag(t) \setminus G(t)} \hypergraph^1_t[g]$.

%$\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} \hypergraph^1_t = $. 


%Running $\AggroYanakakis$ on $\{R_t(G(t)) | t \in \hypernodes_\GHD\}$ annotated with $\Var[Z[g]]$ would result in $\Var[Z_\hypergraph]$.

%From Proposition \ref{proposition:var}, $\Var[Z[g]] \leq |\Join_{F \in \hyperedges_{\hypernodes \setminus G}} \pi_{\hypernodes \setminus G}(R_F \ltimes g)|$. 

%we can define $\oplus$ over $\Var[Z[g]]$'s as $+$. We can also define $\otimes$ as $\times$ over $\Var[Z[g]]$'s since ...
\end{proof}


Now we are ready to prove Theorem \ref{theorem:fhtw}. For each $t \in \hypernodes_\GHD$ of a given GHD $(\GHD, \bag)$, if we replace every sample size $k$ (Line 6 of Algorithm \ref{alg:genericsampler}) for $g$ with $\frac{k}{m}$ where $m = (\epsilon^2 \mu |Q^1|)^{1/|\hypernodes_\GHD|}$, % where $m = \max_{x \in G(\GHD)}|\hypernodes_{\GHD(x)}|$, 
$\Var[Z[g]]$ will increase by $m$ times, while the runtime of \GHDSampler will decrease by $m$ times. Therefore, each annotation in $\Join_{t \in \hypernodes_\GHD} R^{\Var}_t$ will increase by $m^{(1/|\hypernodes_\GHD|) |\hypernodes_\GHD|} = \epsilon^2 \mu |Q^1|$ times. From Proposition \ref{proposition:ghdsampler:variance}, now $\Var[Z_\hypergraph] \leq \epsilon^2 \mu |Q^1| \cdot |Q^1|$. From Proposition \ref{proposition:ghdsampler:time}, the expected runtime for \GHDSampler is now $\DataO(\frac{IN^{fhtw(\GHD, \hypergraph)}}{|Q^1|^{1/|\hypernodes_\GHD|}})$ since $\epsilon$ and $\mu$ are constants. Using Chebyshev's inequality gives us $P(|Z_\hypergraph - |Q^1|| \geq \epsilon |Q^1|) \leq \frac{\Var[Z_\hypergraph]}{\epsilon^2 \E[Z_\hypergraph]} \leq \frac{\epsilon^2 \mu |Q^1|^2}{\epsilon^2 |Q^1|^2} = \mu$, which is an $(1\pm\epsilon)$-approximation of $|Q^1|$.


\redtext{
Note that if $\hypernodes_\GHD$ is a singleton, the expected runtime becomes $\DataO(\frac{AGM(\hypergraph)}{|Q^1|})$. From Example \ref{}, the first GHD gives $\DataO(\frac{N^3}{|Q^1|})$ while the second GHD gives $\DataO(\frac{N^{1.5}}{|Q^1|^{1/3}})$. Therefore, if $|Q^1|$ is large and close enough to $AGM(\hypergraph) = N^3$, using the first GHD is more efficient, with almost $\DataO(1)$ time, while the second GHD has almost $\DataO(N^{0.5})$. If $|Q^1|$ is small as a constant, using the second GHD is more efficient, with $\DataO(N^{1.5})$ time. The first GHD results in $\DataO(N^3)$. The decision boundary is when $|Q^1| = \DataO(N^{\frac{9}{4}})$, both GHDs having $\DataO(N^{\frac{3}{4}})$ time.
}

%then the expected runtime of \GHDSampler is $\DataO()$

\redtext{Can we make estimation for all nodes $t$ that contain $x \in G(\GHD)$ ?? Not independent estimation for each node $t$.}


\fi

==> 06.uniform_GHD.tex <==

\vspace*{-0.2cm}
\section{\rerevision{Uniform Sampling over GHDs}} \label{sec:uniform}

\rerevision{We briefly discuss uniform sampling over GHDs as an extension of \ExactWeight \cite{ExactWeight}, which supports uniform sampling over ayclic joins.
Given an acyclic join query, we can build a GHD $(\GHD, \bag)$ where each node corresponds to an edge in $\hyperedges$, i.e., $\bag(t) = F_t \in \hyperedges : \forall t \in \hypernodes_\GHD$. 
We run the bottom-up DP of \Yan in Lines \ref{alg:simpleaggyan:bottom}-\ref{alg:simpleaggyan:bottomend} of Algorithm \ref{alg:simpleaggyan}, while recursively computing $W(g_t)$ for each $t \in \hypernodes_\GHD$ and $g_t \in R_t$ as follows.}

%\in \hypernodes_\GHD$ corresponds to 

For every $t \in \h$ It initializes $W(g_t) = 1$ for every

==> 98.better.tex <==
\section{Towards Better Complexity} \label{sec:better}


\begin{algorithm} [htb]
\caption{{\GHDSampler}($\hypergraph$ = $(\hypernodes_\hypergraph, \hyperedges_\hypergraph)$, $(\GHD(\hypernodes_\GHD, \hyperedges_\GHD), \bag)$, $\{R_F|F \in \hyperedges_\hypergraph\}$)} \label{alg:ghdsampler}
\small{
    \KwIn{Query hypergraph $\hypergraph$, GHD ($\GHD$, $\bag$), and relations $R_F$ for each $F \in \hyperedges_\hypergraph$}
    
    $S_\GHD \leftarrow \emptyset$ \\
    \ForEach{$t \in \hypernodes_\GHD$}
    {
        $\hypergraph_t \leftarrow (\bag(t), \{\pi_{\bag(t)}(F) | F \in \hyperedges_\hypergraph\})$ \\
        $S_\GHD \leftarrow S_\GHD \cup \GenericSampler(\hypergraph_t, G(t),  \{\pi_{\bag(t)}(R_F) | F \in \hyperedges_{\bag(t)})$ \\
    }
    \Return $\SimpleAggroYanakakis((\GHD, \bag), S_\GHD)$ \\
}
\end{algorithm}


\begin{algorithm} [htb]
\caption{{\SimpleAggroYanakakis}($(\GHD(\hypernodes_\GHD, \hyperedges_\GHD), \bag)$, $\{R_t|t \in \hypernodes_\GHD\}$)} \label{alg:simpleaggro}
\small{
    \KwIn{GHD ($\GHD$, $\bag$) and relations $R_t$ for each $t \in \hypernodes_\GHD$}
    
    \While{$t \in \hypernodes_\GHD$ in some bottom-up order}
    {
        $\beta \leftarrow \{a \in G(t) | TOP_\GHD(a) = t\}$ \\
        $R' \leftarrow \sum_\beta {R_t}$ \\
        
        \If{$t$ is not the root}
        {
            $P \leftarrow $ {parent of} $t$ \\
            $R_P \leftarrow R_P \Join R'$ \\
        }
    }
    
    \Return $R_r$ for the root $r$ \\
}
\end{algorithm}


\begin{algorithm} [htb]
\caption{{\GenericSampler}($\hypergraph = (\hypernodes, \hyperedges)$, $G$, $\{R_F|F \in \hyperedges\}$)} \label{alg:genericsampler}
\small{
    \KwIn{Hypergraph $\hypergraph$, join attributes with other bags $G$, and relations $R_F$ for each $F \in \hyperedges$}
    
    $Z \leftarrow \emptyset$ \\
    
    %Pick $I$ arbitrarily such that $1 \leq |I| < |\hypernodes|$ \\
    %Choose $v$ an arbitrary order of attributes in $\hypernodes \setminus G$ \\
    $\hypergraph_G \leftarrow (G, \{\pi_{G}(F) | F \in \hyperedges_G\})$ \\
    $\hypergraph_{-G} \leftarrow (\hypernodes \setminus G, \{ \pi_{\hypernodes \setminus G}(F) | F \in \hyperedges_{\hypernodes \setminus G} \})$ \\
    $x \leftarrow \text{optimal fractional edge cover of}$ $\hypergraph$ \\
    
    %GenericJoin? EnumerateTuples?
    %\ForEach{$t_G \in \redtext{\EnumerateTuples}(\hypergraph_G, \{\pi_{G}(R_F) | F \in \hyperedges_G\})$}
    \ForEach{$t_G \in \redtext{\GenericJoin}(\Join_{F \in \hyperedges_G} \pi_{G}(R_F))$}

    {
        $Z[t_G] \leftarrow \SamplingEstimator(\hypergraph_{-G}, \{\pi_{\hypernodes \setminus G}(R_F \ltimes t_G) | F \in \hyperedges_{\hypernodes \setminus G}\}, \redtext{k}, x)$ \\
        $Z \leftarrow Z \cup \{(t_G, Z[t_G])\}$ \\
    }
    
    \Return $Z$ \\
}
\end{algorithm}

\iffalse
\begin{algorithm} [htb]
\caption{{\EnumerateTuples}($\hypergraph = (\hypernodes, \hyperedges)$, $\{R_F | F \in \hyperedges\}$)} \label{alg:enumeratetuples}
\small{
    \KwIn{Hypergraph $\hypergraph$ and relations $R_F$ for each $F \in \hyperedges$}
    
    $Q \leftarrow \emptyset$ \\
    
    Pick $I$ arbitrarily such that $|I| = 1$, $I \subset \hypernodes$ \\
    $F^* \leftarrow \argmin_{F \in \hyperedges_I}|R_F|$ \\ %semi-join included
    $\hypergraph_{-I} \leftarrow (\hypernodes \setminus I, \{ \pi_{\hypernodes \setminus I}(F) | F \in \hyperedges_{\hypernodes \setminus I} \})$ \\

    \ForEach{$t_I \in \pi_{I}(R_{F^*})$}
    {
        $Q \leftarrow Q \cup \{t_I\} \times \EnumerateTuples(\hypergraph_{-I}, \{\pi_{\hypernodes \setminus I}(R_F \ltimes t_I) | F \in  \hyperedges_{\hypernodes \setminus I}\})$ \\
    }
    
    \Return $Q$ \\
}
\end{algorithm}
\fi


\begin{algorithm} [htb]
\caption{{\SamplingEstimator}($\hypergraph = (\hypernodes, \hyperedges)$, $\{R_F|F \in \hyperedges\}$, $S$, $\{x_F | F \in \hyperedges\}$, \redtext{$\leaves$})} \label{alg:samplingestimator}
\small{
    \KwIn{Hypergraph $\hypergraph$, relations $R_F$ for each $F \in \hyperedges$, sample size $S$, fractional edge cover $\{x_F\}$, \redtext{and leaf relations $\leaves$}}
    
    Pick $I$ arbitrarily such that $|I| = 1$, $I \subset \hypernodes$ \\
    $F^* \leftarrow \argmin_{F \in \hyperedges_I}|R_F|$ \\ %semi-join included
    \If{$|R_{F^*}| = 0$}
    {
        \Return 0 \\
    }
    
    $\Samples_{I} \leftarrow $ uniform independent samples from $\pi_{I}(R_{F^*})$ with $|\Samples_{I}| = S$ \\
    
    \If{$|\hypernodes| = 1$}
    {
        \Return $\frac{|R_{F^*}|}{|\Samples_I|} \sum_{s_I \in \Samples_I}\I[s_I \in R_F : \forall F \in \hyperedges] \redtext{\prod_{F \in \leaves} |R_F \ltimes s_I|}$ \\
    }
    
    %Pick $I$ arbitrarily such that $1 \leq |I| < |\hypernodes|$ \\
    $\hypergraph_{-I} \leftarrow (\hypernodes \setminus I, \{ \pi_{\hypernodes \setminus I}(F) | F \in \hyperedges_{\hypernodes \setminus I} \})$ \\

    %Arbitrarily order vertices
    
    %$k \leftarrow s \mapsto \ceil{|\pi_{I}(R_{F^*})|  \frac{ \prod_{F \in \hyperedges_{\hypernodes \setminus I} }{|R_F \ltimes s|^{x_F}} }{ \prod_{F \in \hyperedges}{|R_F|^{x_F}} }}$ \\
    $k \leftarrow s \mapsto \ceil{|\pi_{I}(R_{F^*})|  \frac{AGM(\hypergraph_{-I})}{AGM(\hypergraph)}}$ \\
    
    
    \Return $\frac{|\pi_{I}(R_{F^*})|}{|\Samples_I|} \sum_{s_I \in \Samples_I} \I[s_I \in \pi_I(R_F) : \forall F \in \hyperedges_I] \cdot$
    $\SamplingEstimator(\hypergraph_{-I}, \{\pi_{\hypernodes \setminus I}(R_F \ltimes s_I) | F \in \hyperedges_{\hypernodes \setminus I}\}, k(s_I), \{x_F | F \in \hyperedges_{\hypernodes \setminus I}\}, \redtext{\leaves})$ \\
}
\end{algorithm}

Let $Z_\hypergraph$ for the return value of \SamplingEstimator given $\hypergraph$.

\begin{proposition2}\label{proposition:exp}
$\E[Z_\hypergraph] = |\Join_{F \in \hyperedges}R_F|$ for any sample size $S$.
\end{proposition2}

\begin{proof}
Since $\Samples_I$ consists of independent samples, the expectation is the same for all $S$ values. We set $S = 1$ (thus $\Samples_I = \{s_I\}$) and use the proof by induction. 

If $|\hypernodes| = 1$, 

\begin{equation}
\begin{split}
    \E[Z_\hypergraph] &= \sum_{s_I \in R_{F^*}}{P(s_I)} \, |R_{F^*}| \, \I[s_I \in R_F : \forall F \in \hyperedges] \\
    &= \sum_{s_I \in R_{F^*}} \I[s_I \in R_F : \forall F \in \hyperedges] \\
    &= \sum_{s_I \in \cap_{F \in \hyperedges}{R_F}} 1 = |\Join_{F \in \hyperedges} R_F|.
    %&= OUT(\hypergraph, \{R_F|F \in \hyperedges\}).
\end{split}
\end{equation}


If $|\hypernodes| > 1$,

\begin{equation}
\begin{split}
    \E[Z_\hypergraph] &= \sum_{s_I \in \pi_{I}(R_{F^*})}{P(s_I)} \, |\pi_{I}(R_{F^*})| \, \I[s_I \in \pi_{I}(R_F) : \forall F \in \hyperedges_I] \, \E[Z_{\hypergraph_{-I}}] \\
    &= \sum_{s_I \in \pi_{I}(R_{F^*})} \I[s_I \in \pi_{I}(R_F) : \forall F \in \hyperedges_I] \,
    \E[Z_{\hypergraph_{-I}}] \\
    &= \sum_{s_I \in \cap_{F \in \hyperedges_I}{ \pi_{I}(R_{F}) }} |\Join_{F \in \hyperedges_{\hypernodes \setminus I}} \pi_{\hypernodes \setminus I}(R_F \ltimes s_I)| \\
    &= |\Join_{F \in \hyperedges} R_F|.
    %OUT(\hypergraph_{-I}, \{\pi_{\hypernodes \setminus I}(R_F \ltimes s_I) | F \in \hyperedges_{\hypernodes \setminus I}\}) \\
    %&= OUT_\hypergraph.
\end{split}
\end{equation}

\end{proof}


\begin{proposition2}\label{proposition:var}
\Var[Z_\hypergraph] \leq \frac{1}{S} |\hypernodes| \, AGM(\hypergraph) \, |\Join_{F \in \hyperedges} R_F|.
\end{proposition2}

\begin{proposition2}\label{proposition:varopt}
\redtext{\Var[Z_\hypergraph] \leq \frac{1}{S} |\hypernodes_\J| \, AGM(\J) \, |\Join_{F \in \hyperedges} R_F|.}
\end{proposition2}

\begin{proof}
We again use the proof by induction and set $S = 1$. Since $s_I$'s are independent, the variance of $Z_\hypergraph$ is inversely proportional to $S$. Hence, it is enough to show that $\Var[Z_\hypergraph] \leq |\hypernodes| \, AGM(\hypergraph) \, |\Join_{F \in \hyperedges} R_F|$ for $S = 1$.

If $|\hypernodes| = 1$, 

\begin{equation}
\begin{split}
    \Var[Z_\hypergraph] &\leq \E[Z^2_\hypergraph] \\
    &= \sum_{s_I \in R_{F^*}}{P(s_I)} \, |R_{F^*}|^2 \, \I[s_I \in \pi_{I}(R_F) : \forall F \in \hyperedges_I]^2 \\
    &= \sum_{s_I \in R_{F^*}} |R_{F^*}| \, \I[s_I \in \pi_{I}(R_F) : \forall F \in \hyperedges_I] \\
    &= |R_{F^*}| \sum_{s_I \in R_{F^*}} \I[s_I \in \pi_{I}(R_F) : \forall F \in \hyperedges_I] \\
    &= |R_{F^*}| |\Join_{F \in \hyperedges} R_F| \\
    &\leq \prod_{F \in \hyperedges}|R_F|^{x_F} |\Join_{F \in \hyperedges} R_F| \\
    &= AGM(\hypergraph) \, |\Join_{F \in \hyperedges} R_F|.
\end{split}
\end{equation}

If $|\hypernodes| > 1$, $\Var[Z_\hypergraph] &= \E_{s_I}[\Var[Z_\hypergraph|s_I]] + \Var_{s_I}[\E[Z_\hypergraph|s_I]]$ from the law of total variance. We bound the second term first.

\begin{equation}
\begin{split}
    \Var_{s_I}[\E[Z_\hypergraph|s_I]] &= \Var_{s_I}[|\Join_{F \in \hyperedges} (R_F \ltimes s_I)|] \\
    &\leq \E_{s_I}[|\Join_{F \in \hyperedges} (R_F \ltimes s_I)|^2] \\
    &= \sum_{s_I \in \pi_{I}(R_{F^*})}{P(s_I)} \, |\Join_{F \in \hyperedges} (R_F \ltimes s_I)|^2 \\
    &\leq \sum_{s_I \in \pi_{I}(R_{F^*})} |\Join_{F \in \hyperedges} (R_F \ltimes s_I)|^2 \\
    &\leq \Big( \sum_{s_I \in \pi_{I}(R_{F^*})} |\Join_{F \in \hyperedges} (R_F \ltimes s_I)| \Big)^2 \\
    &= \Big( \sum_{s_I \in \pi_{I}(R_{F^*})} \I[s_I] \, |\{s_I\} \times \Join_{F \in \hyperedges_{\hypernodes \setminus I}} \pi_{\hypernodes \setminus I}(R_F \ltimes s_I)| \Big)^2\\
    &= \Big( \sum_{s_I \in \cap_{F \in \hyperedges} \pi_{I}(R_{F})} |\{s_I\} \times \Join_{F \in \hyperedges_{\hypernodes \setminus I}} \pi_{\hypernodes \setminus I}(R_F \ltimes s_I)| \Big)^2\\
    &= |\Join_{F \in \hyperedges} R_F|^2 \leq AGM(\hypergraph) \, |\Join_{F \in \hyperedges} R_F|.
\end{split}
\end{equation}


For the second term,

\begin{equation}
\begin{split}
    \E_{s_I}[\Var[Z_\hypergraph|s_I]] &= \sum_{s_I} P(s_I) \, \Var[Z_\hypergraph|s_I] \\
    &= \sum_{s_I} P(s_I) \, \frac{1}{k(s_I)} \Var[ |\pi_{I}(R_{F^*})| \, \I[s_I] \, Z_{\hypergraph_{-I}}  ] \\
    &= \sum_{s_I} P(s_I) \, \frac{1}{k(s_I)} \, |\pi_{I}(R_{F^*})|^2 \, \I[s_I]^2 \Var[  Z_{\hypergraph_{-I}}  ] \\
    &= \sum_{s_I} \frac{|\pi_{I}(R_{F^*})|}{k(s_I)} \, \I[s_I] \, \Var[  Z_{\hypergraph_{-I}}  ] \\
    &\leq \sum_{s_I} \frac{|\pi_{I}(R_{F^*})|}{k(s_I)} \, \I[s_I] \, |\hypernodes \setminus I| \, AGM(\hypergraph_{-I}) \, |\Join_{F \in \hyperedges_{\hypernodes \setminus I}} \pi_{\hypernodes \setminus I}(R_F \ltimes s_I)| \\
    &\leq \sum_{s_I} \I[s_I] \, |\hypernodes \setminus I| \, AGM(\hypergraph) \, |\Join_{F \in \hyperedges_{\hypernodes \setminus I}} \pi_{\hypernodes \setminus I}(R_F \ltimes s_I)| \\
    &= (|\hypernodes|-1) \, AGM(\hypergraph) \,  |\Join_{F \in \hyperedges} R_F|.
\end{split}
\end{equation}

By adding the upper bounds for the two terms, we have $\Var[Z_\hypergraph] \leq |\hypernodes| \, AGM(\hypergraph) \, |\Join_{F \in \hyperedges} R_F|$ as desired.

\end{proof}

\begin{proof}
\redtext{$\Var_{s_I}[\E[Z_\hypergraph|s_I]]$ is same. $\E_{s_I}[\Var[Z_\hypergraph|s_I]]$ needs to be multiplied by $\prod_{L \in \leaves_{I_{cum}}} |R_F \ltimes s_{I}|$}
\end{proof}

\begin{proposition2}\label{proposition:time}
Expected time for \SamplingEstimator is $\DataO(S)$.
\end{proposition2}

\begin{proof}
We again use the proof by induction. Then, \SamplingEstimator takes expected $\DataO(S) + \sum_{s_I \in \Samples_I} \DataO(k(s_I))$ time at Lines 5 and 10, and $\DataO(1)$ for the other lines, it is enough to show that $k(s_I)$ is expected $\DataO(1)$.

\begin{equation}
\begin{split}
    E_{s_I}[k(s_I)] &= \sum_{s_I \in \pi_{I}(R_{F^*})} P(s_I) \ceil{|\pi_{I}(R_{F^*})|  \frac{AGM(\hypergraph_{-I})}{AGM(\hypergraph)}} \\
    &\leq 1 + \sum_{s_I \in \pi_{I}(R_{F^*})} P(s_I) {|\pi_{I}(R_{F^*})|  \frac{AGM(\hypergraph_{-I})}{AGM(\hypergraph)}} \\
    &= 1 + \sum_{s_I \in \pi_{I}(R_{F^*})} \frac{AGM(\hypergraph_{-I})}{AGM(\hypergraph)} \leq 2 = \DataO(1).
\end{split}
\end{equation}

The last inequality is equivalent to $\sum_{s_I \in \pi_{I}(R_{F^*})} AGM(\hypergraph_{-I}) \leq AGM(\hypergraph)$, which is equivalent to Lemma 1 of \cite{GJSampler}.

\end{proof}

Note that the variance is inversely proportional to $S$, while the expected runtime is proportional to $S$. This variance-runtime trade-off is the key to solve our PAC problem in a desired runtime bound.


\begin{definition2}
\vspace*{-0.2cm}
\label{def:approximation}
For an error bound $\epsilon$, a confidence $\mu \in (0,1)$, and a true value $T$, if the random variable for the estimate $Z$ satisfies $P(\abs{Z-T} \geq \epsilon \cdot T) \leq \mu$, then the estimation is a $(1\pm\epsilon)$-approximation of $T$.
\end{definition2}

\redtext{Need to define $Q^1$, $\hypergraph^1$, $G(\GHD)$, $\GHD(x)$ for an attribute $x$ as the subtree of $\GHD$ of nodes $t$ having $x \in \bag(t)$.}

\begin{theorem}\label{theorem:fhtw}
For arbitrary join query $Q = \hypergraph$ and GHD ($\GHD, \bag$) of $\hypergraph$, $\GHDSampler$ performs $(1\pm\epsilon)$-approximation of $|Q^1|$ in expected \redtext{$\DataO(\frac{IN^{fhtw(\GHD, \hypergraph)}}{|Q^1|^{1/|\hypernodes_\GHD|}})$} time. % where $m = \max_{x \in G(\GHD)} |\hypernodes_{\GHD(x)}|$.
%There exists a randomized algorithm that given a precision parameterε∈(0,1),a subgraphH, and a query access to the input graphG, with high probability outputs a(1±ε)approximation to the number of occurrences ofHinG, denoted by#H, using:
\end{theorem}

The proof for unbiasedness is straightforward. Each call to \SamplingEstimator at Line 6 of Algorithm \ref{alg:genericsampler} returns an unbiased estimate for $\hypergraph_{-G}$ given $t_G$. Therefore, each node $t \in \hypernodes_\GHD$ receives a relation $R_t$ with unbiased estimates for $\sum_{\bag(t) \setminus G(t)} \hypergraph^1_t$ (each tuple in $\hypergraph^1_t$ is a join result of $\hypergraph_t$ with annotation one). As a result, \GHDSampler returns an unbiased estimate of $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} \sum_{\bag(t) \setminus G(t)} \hypergraph^1_t$ = $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \sum_{\cup_{t \in \hypernodes_\GHD} \bag(t) \setminus G(t)} \Join_{t \in \hypernodes_\GHD} \hypergraph^1_t$ = $\sum_{\cup_{t \in \hypernodes_\GHD} \bag(t)} \Join_{t \in \hypernodes_\GHD} \hypergraph^1_t$ = $|Q^1|$.

%$|\hypergraph_t(t_G)|$ as annotations for tuples $t_G$. This is equivalent to $\sum_{\bag(t) \setminus G(t)} R$ where $R = \, \Join_{F \in \hyperedges} R_F$ with all tuple annotations are ones. As a result, \SimpleAggroYanakakis at Line 5 of Algorithm \ref{alg:ghdsampler} is expected to return $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R_t$ = Q.

Therefore, we focus on the variance and runtime. 

\begin{proposition2}\label{proposition:genericsampler:time}
For any $t \in \hypernodes_\GHD$, if we set $k = |\hypernodes| \, AGM(\hypergraph_{-G})$ for each tuple $t_G \in \hypergraph^1_G$, the expected runtime for \GenericSampler is $\DataO(AGM(\hypergraph))$.
\end{proposition2}

\begin{proof}
Line 5 of Algorithm \ref{alg:genericsampler} takes $\DataO(AGM(\hypergraph_G))$ where $AGM(\hypergraph_G) \leq AGM(\hypergraph)$ from the node-monotonicity of $AGM$ \cite{AJAR}.
The expected runtime of Lines 5-7 is $\sum_{t_G \in \hypergraph^1_G} AGM(\hypergraph_{-G}))$ from Proposition \ref{proposition:time}, which is less than $AGM(\hypergraph)$ from the query decomposition lemma of \cite{GenericJoin}.
Since the other lines take $\DataO(1)$, the expected runtime of Algorithm \ref{alg:genericsampler} is $\DataO(AGM(\hypergraph))$ as desired.
\end{proof}


\begin{proposition2}\label{proposition:ghdsampler:time}
For each $t \in \hypernodes_\GHD$ and $\hypergraph_t = (\hypernodes, \hyperedges)$, if we use the same $k$ from Proposition \ref{proposition:genericsampler:time}, the expected runtime for \GHDSampler is $\DataO(IN^{fhtw(\GHD, \hypergraph)})$.
\end{proposition2}

The proof is straightforward. Line 4 of Algorithm \ref{alg:ghdsampler} takes expected $\DataO(\max_{t \in \hypernodes_\GHD} AGM(\hypergraph_t))$ from Proposition \ref{proposition:genericsampler:time}. Line 5 takes $\DataO(IN + OUT)$ \cite{AJAR} where $IN = \DataO(\max_{t \in \hypernodes_\GHD} AGM(\hypergraph_t))$ and $OUT = 1$. Therefore, the expected runtime of \GHDSampler is $\DataO(\max_{t \in \hypernodes_\GHD} AGM(\hypergraph_t)) = \DataO(IN^{fhtw(\GHD, \hypergraph)})$.


\begin{proposition2}\label{proposition:ghdsampler:variance}
For each $t \in \hypernodes_\GHD$ and $\hypergraph_t = (\hypernodes, \hyperedges)$, if we use the same $k$ from Proposition \ref{proposition:genericsampler:time}, $\Var[Z_\hypergraph] \leq |\hypergraph^1|$ (= $|Q^1|$) for the estimate $Z_\hypergraph$ of \GHDSampler.
\end{proposition2}


\begin{proof}
$\Var[Z_\hypergraph] = \Var[\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R_t]$ where $R_t$ is the result of \GenericSampler annotated with $Z[t_{G(t)}]$'s, as in the analysis for the unbiasedness of $Z_\hypergraph$. 

%We can compute $\Var[Z_\hypergraph]$ from $\Var[Z[t_G(t)]]$ (Line 6 of Algorithm \ref{alg:genericsampler}) for each GHD node $t \in \hypernodes_\GHD$.
Since all $Z[t_G]$'s are mutually independent, even across different GHD nodes, $\Var[Z[t_G] + Z[t'_{G}]]$ = $\Var[Z[t_G]] + \Var[Z[t'_{G}]]$ and $\Var[Z[t_G \Join t'_{G'}]]$ = $\Var[Z[t_G] \times Z[t'_{G'}]]$ = $\Var[Z[t_G]] \times \Var[Z[t'_{G'}]]$ for any $t_G$, $t'_{G}$, and $t'_{G'}$ ($G \cap G' \neq \emptyset$). Therefore, as $Z[t_G]$ was the annotation for $t_G$ when estimating $|Q^1|$, we can regard $\Var[Z[t_G]]$ as the annotation for $t_G$ when calculating $\Var[Z_\hypergraph]$. We denote $R^{\Var}_t$ as $R_t$ whose annotations are replaced from $Z[t_G]$'s to $\Var[Z[t_G]]$'s.

\redtext{Need to define $\hypergraph[tuple]$ or $Q[tuple]$.}

We then calculate $\Var[Z_\hypergraph]$ as follows.
$\Var[\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R_t]$ = $\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} R^{\Var}_t$ $\leq$ 
$\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} \sum_{\bag(t) \setminus G(t)} \hypergraph^1_t$ = $|Q^1|$. The inequality holds from Proposition \ref{proposition:var}, $\Var[Z[t_G]] \leq |\Join_{F \in \hyperedges_{\hypernodes \setminus G}} \pi_{\hypernodes \setminus G}(R_F \ltimes t_G)| = \sum_{\hypernodes \setminus G} \hypergraph^1_t[t_G] = \sum_{\bag(t) \setminus G(t)} \hypergraph^1_t[t_G]$.

%$\sum_{\cup_{t \in \hypernodes_\GHD} G(t)} \Join_{t \in \hypernodes_\GHD} \hypergraph^1_t = $. 


%Running $\AggroYanakakis$ on $\{R_t(G(t)) | t \in \hypernodes_\GHD\}$ annotated with $\Var[Z[t_G]]$ would result in $\Var[Z_\hypergraph]$.

%From Proposition \ref{proposition:var}, $\Var[Z[t_G]] \leq |\Join_{F \in \hyperedges_{\hypernodes \setminus G}} \pi_{\hypernodes \setminus G}(R_F \ltimes t_G)|$. 

%we can define $\oplus$ over $\Var[Z[t_G]]$'s as $+$. We can also define $\otimes$ as $\times$ over $\Var[Z[t_G]]$'s since ...
\end{proof}


Now we are ready to prove Theorem \ref{theorem:fhtw}. For each $t \in \hypernodes_\GHD$ of a given GHD $(\GHD, \bag)$, if we replace every sample size $k$ (Line 6 of Algorithm \ref{alg:genericsampler}) for $t_G$ with $\frac{k}{m}$ where $m = (\epsilon^2 \mu |Q^1|)^{1/|\hypernodes_\GHD|}$, % where $m = \max_{x \in G(\GHD)}|\hypernodes_{\GHD(x)}|$, 
$\Var[Z[t_G]]$ will increase by $m$ times, while the runtime of \GHDSampler will decrease by $m$ times. Therefore, each annotation in $\Join_{t \in \hypernodes_\GHD} R^{\Var}_t$ will increase by $m^{(1/|\hypernodes_\GHD|) |\hypernodes_\GHD|} = \epsilon^2 \mu |Q^1|$ times. From Proposition \ref{proposition:ghdsampler:variance}, now $\Var[Z_\hypergraph] \leq \epsilon^2 \mu |Q^1| \cdot |Q^1|$. From Proposition \ref{proposition:ghdsampler:time}, the expected runtime for \GHDSampler is now $\DataO(\frac{IN^{fhtw(\GHD, \hypergraph)}}{|Q^1|^{1/|\hypernodes_\GHD|}})$ since $\epsilon$ and $\mu$ are constants. Using Chebyshev's inequality gives us $P(|Z_\hypergraph - |Q^1|| \geq \epsilon |Q^1|) \leq \frac{\Var[Z_\hypergraph]}{\epsilon^2 \E[Z_\hypergraph]} \leq \frac{\epsilon^2 \mu |Q^1|^2}{\epsilon^2 |Q^1|^2} = \mu$, which is an $(1\pm\epsilon)$-approximation of $|Q^1|$.


\redtext{
Note that if $\hypernodes_\GHD$ is a singleton, the expected runtime becomes $\DataO(\frac{AGM(\hypergraph)}{|Q^1|})$. From Example \ref{}, the first GHD gives $\DataO(\frac{N^3}{|Q^1|})$ while the second GHD gives $\DataO(\frac{N^{1.5}}{|Q^1|^{1/3}})$. Therefore, if $|Q^1|$ is large and close enough to $AGM(\hypergraph) = N^3$, using the first GHD is more efficient, with almost $\DataO(1)$ time, while the second GHD has almost $\DataO(N^{0.5})$. If $|Q^1|$ is small as a constant, using the second GHD is more efficient, with $\DataO(N^{1.5})$ time. The first GHD results in $\DataO(N^3)$. The decision boundary is when $|Q^1| = \DataO(N^{\frac{9}{4}})$, both GHDs having $\DataO(N^{\frac{3}{4}})$ time.
}

%then the expected runtime of \GHDSampler is $\DataO()$

\redtext{Can we make estimation for all nodes $t$ that contain $x \in G(\GHD)$ ?? Not independent estimation for each node $t$.}


\subsection{TDs with Binary Relations} \label{subsec:TD}

\subsection{Binary Degree Constraints} \label{subsec:degree}





==> 99.randomwalk.tex <==
\section{Random Walk with Dynamic Ordering} \label{sec:randomwalk}

We use random walk where the sampling order of query vertices is dynamically determined. This is a novel approach in constrast to previous methods \cite{SSTE, Alley, GenericJoin} that use a fixed order. %Not only \SSTE and \Alley, worst-case optimal join algorithms or subgraph enumeration algorithms
With a simple heuristic, we show that the dynamic ordering bounds the variance as in Table \ref{table:summary}.

Our \GenericSampler (Algorithm \ref{alg:main}) implements (\ref{eq:decomposition2}) and works for an arbitrary labeled graph $H$. 

\redtext{우선 알고리즘 제시 as an instantiation of (4), Sampler Tree는 이 알고리즘의 virtual output. (4)의 Sample Space는 어떻게 계산되는지, Samples S는 뭐에 대응되는지, Y, t, u, v, w...}

% 실제 구현 때는 Sample Space 한번 구하고 여러번 sample하면 됨

\iffalse
\begin{algorithm} [htb]
\caption{{\Sampler}($H, G, x, i, L$)} \label{alg:main}
\small{
    \KwIn{A query graph $H$, a data graph $G$ of binary tables $\{R\}$, recursion depth $i$, a half-integral optimal fractional edge cover $x$ of $H$, and current sample $L: V(L) \rightarrow V(G)$ where $V(L) \subseteq V(H)$ and $|V(L)| = i-1$}
    
    $E(L) \leftarrow \{(u, u') \in E(H) \,|\, u, u' \in V(L)\}$ \\
    \redcomment{Dynamically choose the query vertex}
    $(u^*, e^*) \leftarrow \argmin_{(u, e) \, \text{s.t.} \, u \in V(H) \setminus V(L), \, e \in E(H) \setminus E(L) \, e \ni u}{|R_e \ltimes L|}$ \\
    
    \redcomment{Sample a data vertex}
    $\SampleSpace \leftarrow \pi_{u^*}(R_{e^*} \ltimes L)$ \\
    \If{$\SampleSpace = \emptyset$}
    {
        \Return 0 \\
    }
    
    $v^* \sim \SampleSpace$ \\
    $L^* \leftarrow L \cup \{u^* \mapsto v^*\}$ \\
    
    \If{$i = n$}
    {
        \Return $\frac{1}{|\SampleSpace|} \cdot \I[L^* \in \Matches]$ \\
    }
    
    %$V = \{v_1, v_2, ..., v_t\} \sim \SampleSpace$ \\

    \redcomment{Recursion}
    $E(L^*) \leftarrow E(L) \cup \{(u, u^*) \in E(H) \,|\, u \in V(L)\}$ \\
    $t \leftarrow \ceil{|\SampleSpace| \cdot \frac{ \prod_{e \in E(H) \setminus E(L^*)}{|R_e \ltimes L^*|^{x_e}} }{ \prod_{e \in E(H) \setminus E(L)}{|R_e \ltimes L|^{x_e}} }}$ \\

    $Y \leftarrow 0$ \\
    \ForEach{$j \in [t]$}
    {
        $Y^* \leftarrow \Sampler(H, G, x, i+1, L^*)$ \\
        $Y \leftarrow Y + Y^*$ \\
    }
    $Y \leftarrow \frac{1}{|\SampleSpace| \cdot t} \cdot Y$ \\
    
    \Return $Y$ \\
}
\end{algorithm}
\fi


\begin{algorithm} [htb]
\caption{{\GenericSampler}($H, G, k$)} \label{alg:main}
\small{
    \KwIn{A query graph $H$, a data graph $G$ of binary tables $\{R\}$, and the number of sampling units $k$}
    
    $x \leftarrow \HalfIntegralCover(H, G)$ \\
    
    $(u_1, e_1) \leftarrow \argmin_{(u, e) \, \text{s.t.} \, u \in V(H), \, e \in E(H), \, e \ni u}{|R_e|}$ \\
    $\SampleSpace_1 \leftarrow \pi_{u_1}(R_{e_1})$ \\
    
    $\Samples_1 \leftarrow \SampleFrom(\SampleSpace_1, k)$ \\
    
    $Z \leftarrow 0$ \\
    \ForEach{$v_1 \in \Samples_1$}
    {
        $L_1 \leftarrow \{u_1 \mapsto v_1\}$ \\
        $t_1 \leftarrow \ceil{|\SampleSpace_1| \cdot \frac{ \prod_{e \in E(H)}{|R_e \ltimes L_1|^{x_e}} }{ \prod_{e \in E(H)}{|R_e|^{x_e}} }}$ \\
        $Y_1 \leftarrow \RecursiveSampler(H, G, x, 1, |\SampleSpace_1|, t_1, L_1)$ \\
        $Z \leftarrow Z + Y_1$ \\
    }
    $Z \leftarrow \frac{Z}{k}$ \\
    
    \Return $Z$ \\
}
\end{algorithm}


\begin{algorithm} [htb]
\caption{{\RecursiveSampler}($H, G, x, i, w_i, t_i, L_i$)} \label{alg:recursive}
\small{
    \KwIn{A query graph $H$, a data graph $G$ of binary tables $\{R\}$, a half-integral optimal fractional edge cover $x$ of $H$, current recursion depth $i$, sampling weight for current step $w_i$, sample size $t_i$, and current sample $L_i: V_i \rightarrow V(G)$ where $V_i \subseteq V(H)$ and $|V_i| = i$}
    
    \If{$i = |V(H)|$}
    {
        \Return $w_i \cdot \I[L_i \in \Matches]$ \\
    }
    
    $E_i \leftarrow \{(u, u') \in E(H) \,|\, u, u' \in V_i\}$ \\
    $(u_{i+1}, e_{i+1}) \leftarrow \argmin_{(u, e) \, \text{s.t.} \, u \in V(H) \setminus V_i, \, e \in E(H) \setminus E_i \, e \ni u}{|R_e \ltimes L_i|}$ \\
    $\SampleSpace_{i+1} \leftarrow \pi_{u_{i+1}}(R_{e_{i+1}} \ltimes L_i)$ \\
    \If{$\SampleSpace_{i+1} = \emptyset$}
    {
        \Return 0 \\
    }
    $E_{i+1} \leftarrow \{(u, u') \in E(H) \,|\, u, u' \in V_i \cup \{u_{i+1}\}\}$ \\
    $\Samples_{i+1} \leftarrow \SampleFrom(\SampleSpace_{i+1}, t_i)$ \\

    $Y_{i} \leftarrow 0$ \\
    \ForEach{$v_{i+1} \in \Samples_{i+1}$}
    {
        $L_{i+1} \leftarrow L_i \cup \{u_{i+1} \mapsto v_{i+1}\}$ \\
        $t_{i+1} \leftarrow \ceil{|\SampleSpace_{i+1}| \cdot \frac{ \prod_{e \in E(H) \setminus E_{i+1}}{|R_e \ltimes L_{i+1}|^{x_e}} }{ \prod_{e \in E(H) \setminus E_i}{|R_e \ltimes L_i|^{x_e}} }}$ \\
        $Y_{i+1} \leftarrow \RecursiveSampler(H, G, x, i+1, |\SampleSpace_{i+1}|, t_{i+1}, L_{i+1})$ \\
        $Y_i \leftarrow Y_i + Y_{i+1}$ \\
    }
    $Y_i \leftarrow \frac{w_i}{t_i} \cdot Y_i$ \\
    
    \Return $Y_i$ \\
}
\end{algorithm}



We extend sampler tree used in \cite{SSTE} to explain our algorithm.  

\begin{definition2}
\label{def:samplertree}
A sampler tree $\SamplerTree$ is a triple $(u, v, w)$ where each element is a function from each tree node to $V(H)$, $V(G)$, and $\mathbb{R}$, respectively. 
For any path $p = \gamma \rightarrow \alpha$ from the root $\gamma$ to a node $\alpha$, $u$ is injective, i.e., $u(a) = u(b)$ iff $a = b$ for any $a, b \in p$. $\cup_{\beta \in p}{\{u(\beta) \mapsto v(\beta)\}}$ corresponds to a sample of $H'$, the subgraph of $H$ projected onto $\cup_{\beta \in \gamma \rightarrow \alpha}{\{u(\beta)\}}$, in $G$. $w(\alpha)$ is the weight of $\alpha$, the inverse of probability sampling $v(\alpha)$ given the nodes from $\gamma$ to $Parent(\alpha)$, the parent of $\alpha$.
%For any node $\alpha \in \SamplerTree$, the path from the root to $\alpha$
%For node $\alpha$, $Parent(\alpha)$ and $Child(\alpha)$ denote the parent and children of $\alpha$, respectively. $L_\alpha$ and $ $
Here, $L_\alpha$ = $\cup_{\beta \in \gamma \rightarrow Parent(\alpha)}{\{u(\beta) \mapsto v(\beta)\}}$ is called the prefix or condition of $\alpha$.
\end{definition2}

The tree nodes $\{\alpha\}$ at depth $i$ may have different $u(\alpha)$ values, to capture the dynamic ordering of query vertices. The original tree in \SSTE can be defined as a pair $(v, w)$ without $u$ from the fixed ordering, and $v$ and $w$ are functions from components, not vertices. \redtext{Figure \ref{} shows an example of $\SamplerTree$. If the depth of a node is $n-1$, we call it a leaf node. A path from the root may not reach a leaf node as ... if the sample space $\SampleSpace_{i+1}$ for a node $\alpha$ of depth $i$ (< $n$) becomes empty, so $v$ cannot map $\alpha$ to a data vertex.}


We define two additional random variables $Y_\alpha$ and $t_\alpha$ for each node $\alpha$. First, $Y_\alpha$ is recursively defined as follows, corresponding to a partial sum of (\ref{eq:decomposition2}).

\begin{equation}
Y_\alpha = \begin{cases}
w(\alpha) \cdot \I[L_\alpha \cup \{u(\alpha) \mapsto v(\alpha)\} \in \Matches] & \text{$\alpha$ is a leaf} \\
\frac{w(\alpha)}{t_\alpha} \sum_{c \in Child(\alpha)}{Y_c} &\text{$\alpha$ is non-leaf}
\end{cases}
\end{equation}

$Y_\alpha$ (or $Y_\alpha|L_\alpha$) represents the estimate of $(\#H|L_\alpha)$, which is the number of embeddings of $H$ in $G$ with $L_\alpha$ given. That is, we count the embeddings that are supersets of $L_\alpha$, regarding $(u(\beta))_{\beta \in \gamma \rightarrow Parent(\alpha)}$ as free variables.

$t_\alpha$ is the branch size, or number of children of $\alpha$, $|Child(\alpha)|$. It is carefully determined after $L_\alpha \cup \{u(\alpha) \mapsto v(\alpha)\}$ is given, which we explain during the proof of Proposition \ref{proposition:var}. 


The following three propositions explain the unbiasedness, bounded variance, and bounded time complexity of our algorithm, respectively.


\begin{proposition2}\label{proposition:exp}
\E[Y_\gamma] = \#H.
\end{proposition2}

\begin{proof}
It can be proven from (\ref{eq:decomposition2}) where $Y_\gamma$ is the random variable for $\widehat{\#H}$, and $Y_\gamma$  
\end{proof}


\begin{proposition2}\label{proposition:var}
\Var[Y_\gamma] \leq n \cdot AGM(H) \cdot \#H.
\end{proposition2}


\begin{proposition2}\label{proposition:time}
Building a sampler tree $\SamplerTree$ takes expected $O^*(1)$ time.
\end{proposition2}




==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> dynamic.tex <==
\vspace{-0.3cm}

\section{Dynamic Ordering}\label{sec:dynamic}

This section provides an optimization technique, \emph{dynamic ordering}, to further decrease the sample space to increase the accuracy of \Alley.

In Algorithm \ref{alg:alley_sample}, the size of the local sample space, $\abs{P_{o_i}}$, is bounded to the size of the minimum set to be intersected, which is $\min_{e \in E, e \ni o_i}$ $\abs{\pi_{o_i}(F_e \,|\, p)}$. To reduce this bound, we dynamically choose $o_i$ as follows.

\vspace{-0.3cm}
%\begin{equation}\label{eq:dynamic}
\[
o_i = \left\{
\begin{array}{ll}
     \argmin_{ \substack{ u \in U } }{\min_{ \substack{e \in E \\ e \ni u} }\abs{\pi_{u}(F_e)}} & i = 1 \\
     \argmin_{ \substack{u \in U \\ \exists j < i \, \textrm{s.t.} \, (o_j, u) \in E } }{\min_{ \substack{e \in E \\ e \ni u} }\abs{\pi_{u}(F_e \,|\, p)}} & i > 1
\end{array}
\right.
\]
%\end{equation}

%\begin{equation}\label{eq:dynamic}
%o_i = \argmin_{ u \in U, \exists j < i \, \textrm{s.t.} \, (o_j, u) \in E  }{\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e \ltimes p)}}
%\end{equation}

First, we choose $o_1$, the first query vertex to sample for, as $u$ that has an incident edge $e$ whose $\pi_u(F_e)$ is the minimum among all query vertices. 
For subsequent $o_i$ $(i > 1)$, among all query vertices that are connected to an already sampled vertex, we choose the $u$ with the smallest $\min_{e \in E, e \ni u}$ $\abs{\pi_{u}(R_e \,|\, p)}$ before Line 1 in Algorithm \ref{alg:alley_sample}. The dynamic ordering tries to reduce the upper bound of each local sample space $P_{o_i}$, and thus reduces the size of the sample space, $\abs{\SampleSpace}$. We show how the dynamic ordering significantly increases the accuracy in Section \ref{sec:exp}.

In addition, dynamic ordering adds only a small amount of overhead in \Alley since we can obtain each $\abs{\pi_u(F_e \,|\, p)}$ in $O(1)$ time.
Furthermore, recall that each intersection has time complexity $O(\min_{e \in E, e \ni o_i}$ $\abs{\pi_{o_i}(R_e \,|\, p)})$ (see Section \ref{subsec:multiway}), proportional to the minimum size of $\abs{\pi_{o_i}(F_e \,|\, p)}$. 
Hence, the dynamic ordering reduces this size and often increases the efficiency of \Alley. %We also show such cases in Section \ref{sec:exp}.


%reduce the computation overhead of \Alley and further increase the accuracy. 

%While mulit-way intersection significantly increases the accuracy, it's not a free lunch. It is the main bottleneck of \Alley and limits the efficiency as in typical worst-case optimal algorithms \cite{mhedhbi2019optimizing}. %We show in Section \ref{sec:exp} that this intersection is the main bottleneck in \Alley. 
%As in such worst-case optimal algorithms, the multi-way intersection is implemented to run in $O(\min_{e \in E, e \ni o_i}$ $\abs{\pi_{o_i}(R_e \ltimes p)})$ time, proportional to the size of the minimum relation to intersect, in Line 5 of Algorithm \ref{alg:main}.
%The multi-way intersection has time complexity of $O(d(o_i) \cdot \min_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)})$ in Line 5 of Algorithm \ref{alg:main} \cite{}. Here, $d(o_i)$ is the degree of $o_i$ in $\QueryGraph$, the number of relations to intersect.
%Thus the time complexity is linear to both the number of relations to intersect, and the minimum size among this relations.
%However, it is highly likely that $e^* = \argmin_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)}$ is connected to any of precedent vertices of $o_i$, since otherwise $\abs{\pi_{o_i}(R_e \ltimes p)} = \abs{\pi_{o_i}(R_e)}$.
%In addition, the size of the local sample space for $o_i$ is bounded to $\min_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)}$ due to the intersection. %Thus $\min_{e \in E, e \ni o_i}\abs{\pi_{o_i}(R_e \ltimes p)}$ acts as an upper bound of the size of local sample space.

%Therefore, to reduce both the intersection cost and the size of local sample space, we dynamically choose $o_i$ as follows.
%\begin{equation}\label{eq:dynamic}
%o_i = \argmin_{ u \in U, u \not\in \cup_{j<i}{\{u\}} }{\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e \ltimes p)}}
%\end{equation}

%We call this dynamic ordering, and show that this idea greatly increases the accuracy and mitigate the low efficiency problem of \Alley in Section \ref{sec:exp}.

We explain how dynamic ordering works with the running example in Figure \ref{fig:alley}. %The fourth row in Figure \ref{fig:running-example}d shows two sampling orders that are dynamically determined.
First, in Line 1 of Algorithm \ref{alg:main}, we do not fix the whole $o$ but choose $o_1$ as $u_1$, since $u_1$ has an incident edge $(u_1, u_3)$ where $F_{(u_1, u_3)}$ $ = 12$ is the minimum among all $F_e$ $(e \in E)$. Then $P_{o_1} = \{v_1, v_{24}\}$ as before (Figure \ref{fig:alley}b). Assume that $v_1$ is sampled for $u_1$. Then, in the next recursive call to \SamplePotentialEmbeddings\xspace, we choose $o_2 = u_3$ since $\abs{\pi_{u_3}(F_{(u_1, u_3)} \,|\, p)} = 1$ while $\abs{\pi_{u_2}(F_{(u_1, u_2)} \,|\, p)} = 11$, $\abs{\pi_{u_2}(F_{(u_2, u_3)} \,|\, p)} = 1000$ and $\abs{\pi_{u_3}(F_{(u_2, u_3)} \,|\, p)}$ $ = 1000$. Since $P_{o_2} = P_{u_3} = \{v_2\}$ (Figure \ref{fig:alley}j and k), we sample $v_2$ for $u_3$ (Figure \ref{fig:alley}l). Finally, $o_3$ is then chosen as $u_2$, where $P_{u_2} = \{v_{13}\}$ (Figure \ref{fig:alley}m and n). Therefore, if we sample $v_1$ for $u_1$, $m_1$ can be directly sampled. The return value of each recursive call is represented in Figure \ref{fig:alley}o.
If we sample $v_{24}$ for $u_1$, $o_2 = u_2$ and $o_3 = u_3$; $m_2$ can be directly sampled through a similar process. Therefore, $\SampleSpace = \{m_1, m_2\} = \Matches$ which is the minimal possible. Each potential embedding $p \in \SampleSpace$ has probability 1/2 to be sampled, and Equation \ref{eq:variance} gives that the estimation variance is zero, achieving optimal accuracy for this example.

%$V_{o_1} = \{v_0\}$ so we sample $v_0$ for $u_0$ and append it to $p$. Then, we choose $o_2 = u_1$ since $\abs{\pi_{u_1}(R_{(u_1, u_0)} \ltimes p)} = 1$ which is the minimum. $V_{o_2} = \{v_1\}$ so we sample $v_1$ for $u_1$. Similarly, we sample $v_2$ for $o_3 = u_2$ and $v_3$ for $o_4 = u_3$. 
%Note that we used the same $o_1$ to $o_4$ in Section \ref{subsec:overview} when explaining \Alley without dynamic ordering.
%Note that $o_1$ to $o_4$ are same without dynamic ordering in Section \ref{subsec:overview}.
%However, $o_5$ is different that $o_5$ is $u_5$, not $u_4$ (overlined in Figure \ref{fig:running-example}d). This is because $\pi_{u_4}(R_{(u_4, u_0)} \ltimes p) = \{v_4, v_5, v_{16}, v_{17}, ..., v_{113}\}$, $\pi_{u_4}(R_{(u_4, u_3)} \ltimes p) = \{v_4, v_5, v_{115}, v_{116}, ..., v_{212}\}$, and $\pi_{u_4}(R_{(u_4, u_5)} \ltimes p) = \{v_4, v_5, v_6, v_7, v_9, ...\}$, while $ \pi_{u_5}(R_{(u_5, u_8)} \ltimes p)$ is only $\{v_6, v_7\}$.

%Since $V_{o_5} = \{v_6, v_7\}$, we first assume that $v_6$ is sampled for $o_5 = u_5$.
%Now we choose $o_6 = u_4$ since $\abs{\pi_{u_4}(R_{(u_4, u_5)} \ltimes p)} = 1$. After that, we choose $o_7 = u_6$, $o_8 = u_7$, $o_9 = u_8$, and $o_{10} = u_9$ (first order in the fourth row of Figure \ref{fig:running-example}d), sampling the actual embedding $m_1$ of $\QueryGraph$. The probability of sampling this $m_1$ is $\frac{1}{2}$ since $\abs{V_{o_5}} = 2$ and $\abs{V_{o_i}} = 1$ for $i \not\eq 5$.

%However, if we sample $v_7$ instead of $v_6$ for $o_5 = u_5$, the order changes to the second one in the fourth row of Figure \ref{fig:running-example}d. We choose $o_7 = u_7$ instead of $u_6$ (underlined) since $\pi_{u_7}(R_{(u_7, u_5)} \ltimes p) = \{v_{10}\}$ while $\pi_{u_6}(R_{(u_6, u_5)} \ltimes p) = \{v_{11}, v_{311}, ..., v_{409}\}$. We eventually sample $m_2$ with probability $\frac{1}{2}$, because $\abs{V_{o_5}} = 2$ and $\abs{V_{o_i}} = 1$ for $i \not\eq 5$ again.

%Without dynamic ordering, we randomly chose 
%It is clear that $\Matches = \SampleSpace$, achieving zero variance by Equation (\ref{eq:variance}) in Section \ref{subsec:samplespace}. Thus this example shows a case where dynamic ordering leads to an optimal accuracy.

\iffalse

Algorithm \ref{alg:opt} shows how we can lightly incorporate this idea in \Alley. If we na\"ively calculate (\ref{eq:dynamic}) and determine $o_i$, it will take $O(\sum_{ u \in U, u \not\in \cup_{j<i}{\{o_j\}} }d(u))$ time.
%; the first term for updating $R_e \ltimes p$ for each incident edge $e$ of $o_{i-1}$, and the second term for calculating (\ref{eq:dynamic}).
Instead, we can determine $o_i$ in $O(d(o_{i-1}))$ time. First, we maintain the order of query vertices $\{u\}$ sorted by $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e)}$ (Line 1). This determines $o_1$. Then, for each recursive function with $i > 1$, we determine $o_i$ by comparing the $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e \ltimes p)}$ of $u = s_c$ and for each $(o_{i-1}, u) \in E$ such that $u$ has not been sampled (Lines 6-12). Here, $c$ is the cursor for a candidate query vertex $s_c$ whose $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e)}$ is the minimum among all unsampled query vertices. 
If $s_c$ is chosen as $o_i$, increase $c$ until we find the next unsampled query vertex in $s$ (Lines 13-16).


%The overhead of multi-way intersection. Worst-case optimal subgraph matching algorithms use intersection with cost $O(N * min R_e)$. Thus, it is linear to the minimum-size relation. However, this is likely to be $R_e \ltimes p$ with $p \cup e > 0$, so consider the minimum among $R_e \ltimes p$ such that $p \cup e > 0$.

%Rather than choosing the fixed order, dynamically order that seems to reduce the local sample space well.

%Size of local sample space is at most $R_e \ltimes p$, so we choose $min R_e \ltimes p$.

\begin{algorithm} [htb]
\caption{{\Alley}($V, E, R$)} \label{alg:opt}
\small{
    $s \leftarrow $ an order of query vertices $\{u\}$ sorted by $\min_{e \in E, e \ni u}\abs{\pi_{u}(R_e)}$ \\
    $o \leftarrow \emptyset$ \\
    $p \leftarrow \emptyset$ \\
    $w \leftarrow \emptyset$ \\
    \Return \Recursive($V, E, R, o, s, 2, p, w, 1$) \\
    \nonl\Fn{\FMain{\Recursive($V, E, R, o, s, c, p, w, i$)}}{
        \If{$i > 1$}
        {
            $min \leftarrow \min_{e \in E, e \ni s_c}\abs{\pi_{s_c}(R_e)}$ \\
            $o_i \leftarrow s_c$ \\
            \ForEach{$(o_{i-1}, u) \in E$ s.t, $u \not\in \cup_{j<i}{\{o_j\}}$}
            {
                \If{$min > \abs{\pi_{u}(R_{(o_{i-1}, u)} \ltimes p)}$}
                {
                    $min \leftarrow \abs{\pi_{u}(R_{(o_{i-1}, u)} \ltimes p)}$ \\
                    $o_i \leftarrow u$ \\
                }
            }
            \If{$s_c = o_i$}
            {
                \Repeat{$s_c \in \cup_{j \leq i}{\{o_j\}}$}{$c \leftarrow c + 1$}%\Until
            }
        }
        Lines 5-20 in Algorithm \ref{alg:main} with additional parameters $s$ and $c$ for \Recursive
    }
}
\end{algorithm}

\fi

The dynamic ordering does not violate the probabilistic guarantees of \Alley in Section \ref{sec:proof}.
It only adds query related overhead so we can ignore it in the time complexity of \Alley as mentioned in Section \ref{subsec:agm}. %The proofs of lemmas and propositions in Section \ref{sec:proof} are not violated with the random variables we defined; we did not assume the fixed $o$ during the proofs.

Surprisingly, the idea of dynamic ordering has not been considered in existing worst-case optimal subgraph matching algorithms \cite{kankanamge2017graphflow, aref2015design, aberger2016emptyheaded, mhedhbi2019optimizing} while any of these algorithms may adopt this idea in order to reduce the intermediate results size. In detail, if we replace sampling with exhaustive search, %as in the proof of Proposition \ref{lemma:3}, 
$o$ becomes the matching order and the local sample space $P_{o_i}$ becomes the local search space for $o_i$. Therefore, the search space as well as the intermediate results size can be reduced.
